Properly learning monotone functions via local reconstruction

We give a $2^{\tilde{O}(\sqrt{n}/\epsilon)}$-time algorithm for properly learning monotone Boolean functions under the uniform distribution over $\{0,1\}^n$. Our algorithm is robust to adversarial label noise and has a running time nearly matching that of the state-of-the-art improper learning algorithm of Bshouty and Tamon (JACM '96) and an information-theoretic lower bound of Blais et al (RANDOM '15). Prior to this work, no proper learning algorithm with running time smaller than $2^{\Omega(n)}$ was known to exist. The core of our proper learner is a \emph{local computation algorithm} for sorting binary labels on a poset. Our algorithm is built on a body of work on distributed greedy graph algorithms; specifically we rely on a recent work of Ghaffari (FOCS'22), which gives an efficient algorithm for computing maximal matchings in a graph in the LCA model of Rubinfeld et al and Alon et al (ICS'11, SODA'12). The applications of our local sorting algorithm extend beyond learning on the Boolean cube: we also give a tolerant tester for Boolean functions over general posets that distinguishes functions that are $\epsilon/3$-close to monotone from those that are $\epsilon$-far. Previous tolerant testers for the Boolean cube only distinguished between $\epsilon/\Omega(\sqrt{n})$-close and $\epsilon$-far.

==> Monotone corrector new arxiv version/abstract.tex <==
\begin{abstract}
    We give a $2^{\tilde{O}(\sqrt{n}/\eps)}$-time algorithm for properly learning monotone Boolean functions under the uniform distribution over $\{0,1\}^n$. Our algorithm is robust to adversarial label noise and has a running time nearly matching that of the state-of-the-art improper learning algorithm of Bshouty and Tamon (JACM '96) and an information-theoretic lower bound of Blais et al (RANDOM '15). Prior to this work, no proper learning algorithm with running time smaller than $2^{\Omega(n)}$ was known to exist.
    
    The core of our proper learner is a \emph{local computation algorithm} for sorting binary labels on a poset. Our algorithm is built on a body of work on distributed greedy graph algorithms; specifically we rely on a recent work of Ghaffari (FOCS'22), which gives an efficient algorithm for computing maximal matchings in a graph in the LCA model of Rubinfeld et al and Alon et al (ICS'11, SODA'12). The applications of our local sorting algorithm extend beyond learning on the Boolean cube: we also give a tolerant tester for Boolean functions over general posets that distinguishes functions that are $\eps/3$-close to monotone from those that are $\eps$-far. 
    Previous tolerant testers for the Boolean cube only distinguished between 
    $\eps/\Omega(\sqrt{n})$-close and $\eps$-far.
    
\end{abstract}

==> Monotone corrector new arxiv version/correction_algorithm.tex <==
\section{The LCA for poset sorting}
\label{sec:sorting}
In this section, we prove \Cref{thm: the local corrector for general posets}. First, we give a ``global'' algorithm for the poset sorting problem, which reads all the values of $f$ and writes all the values of $f_{mon}$. The global algorithm is inefficient, but lends itself easily to a proof of correctness. We prove correctness for the global algorithm, then give our local implementation and show that it simulates the global algorithm.

\subsection{A global view} 
\label{subsection: the global view}
We first present~\Cref{alg:global}, which sorts the labels of $f$ in stages by swapping the labels of pairs of vertices that violate monotonicity. We will show that each stage reduces the maximum distance between violated vertices by a factor of 2, which produces a monotone function after $\log h$ stages, where $h$ is the height of the input graph.

Before we present the algorithm, we define the following objects that it constructs during its execution.

\begin{definition}[Violation set]
We define the set of violated pairs $\mathrm{viol}_P(f)$ as follows:
\begin{align*}
    &\viol_P(f) := \\ &\{(v, w) \in P \times P : ~ v \succ w,~ f(v)=0 \text{ and } f(w)=1\}.
\end{align*}
\end{definition}

\begin{definition}[$k$-violation graph]
\label{def:viol-graph}
For a poset $P$ of height $h$, a function $f~:~P\to \zo$, and some $k \in [h]$, we define the $k$-violation graph $B_k$ as follows:

\begin{itemize}
	\item $V(B_k) = P$, and 
	\item For $(v, w) \in \mathrm{viol}_P(f)$, $(v, w) \in E(B_k)$ iff $\dist(v,w) \ge k$. 
	%\blue{Arsen: maybe keep the definition the same after all, and introduce the $2k$ thing as an implementation detail in later section? This will let us keep the section unedited}
\end{itemize}
Note that $B_k$ is bipartite and undirected.
\end{definition}

\begin{algorithm}[H]
\begin{algorithmic}
\State \textbf{Given:} Poset $P$ of height $h$, function $f_0:~P \to \zo$
\State \textbf{Output:} monotone function over $P$
\State Let $i \gets 0$
\For{$0 \le i \le \lceil \log h \rceil + 1$}
\State Let $k \gets \lceil h/2^{i+1} \rceil$
\State Construct the $k$-violation graph $B_k$ from $P$ and $f_i$.
%. 
%as defined in \Cref{def:restricted-TC}
\State Compute a maximal matching in $B_k$ and let $\lambda$ map matched vertices to each other, and unmatched vertices to themselves. 
%$\lambda \gets \textsc{MaxMatching}(P_d)$
\State For all $x \in P$, let $f_{i+1}(x) = f_i(\lambda(x))$
\State $i \gets i + 1$
\EndFor
\State \Return $f_i$
\end{algorithmic}
\caption{LCA for sorting labels in a poset: the global view}
\label{alg:global}
\end{algorithm}


\subsection{Correctness of \Cref{alg:global}}
Recall that we are required to show that our algorithm outputs a monotone function that can be obtained from $f$ by a sequence of monotonicity-violating label swaps.
Since it is evident from the pseudocode that this algorithm only performs such swaps, it remains to show only that the output is monotone.
%, that the output differs from $f_0$ by at most twice its distance to monotonicity, and that the algorithm preserves distance to all monotone functions (as required by \Cref{thm: the local corrector for general posets}). 

\input{path_shortening_general}

The following invariant, which will be useful for proving that the output is monotone, is a consequence of \Cref{lemma: path shortening lemma}.

\begin{corollary}[Distance shortening invariant]
\label{claim:distance-invariant}
The following holds for all $f_i$, $0 \le i \le \lceil \log h \rceil$:
$$
\max_{(v, w) \in \viol_P(f)} \dist(v, w) \leq \bigg \lceil \frac{h}{2^i} \bigg \rceil
$$
\end{corollary}

\begin{proof}
We proceed by induction on $i$. For $i=0$, the distance must be at most $h$, because $h$ is the height of $P$. Assume as an inductive hypothesis that the claim holds for some $i \le \lceil \log h \rceil$.

$B_k$ is a graph with the properties described in~\Cref{def:viol-graph}: it has an edge joining each pair of vertices in $P$ that violates monotonicity and has distance at least $k$, for $k = \lceil h / 2^{i+1} \rceil$. By the inductive hypothesis, all such distances are between $\lceil h/2^{i+1}\rceil $ and $\lceil h/2^i \rceil$ inclusive. Then by~\Cref{lemma: path shortening lemma} we guarantee that 
\begin{align*}
&\max_{(v, w) \in \viol_P(f)} \dist(v, w) \\
&\leq \max \bigg (\bigg\lceil \frac{h}{2^{i+1}} \bigg\rceil - 1,  ~ \bigg\lceil \frac{h}{2^i} \bigg\rceil - \bigg\lceil \frac{h}{2^{i+1}}\bigg\rceil \bigg ) \\
&\le \bigg\lceil \frac{h}{2^{i+1}}\bigg\rceil .
\end{align*}
This completes the induction.
\end{proof}
With~\Cref{claim:distance-invariant} in hand, we continue with the proof of correctness.

\begin{lemma}[Correctness]
		\label{lem:correctness}
For any Boolean function $f_0$, poset $P$, and any choice of maximal matchings over $B_k$ in \Cref{alg:global}, the output $f_{\lceil \log h \rceil + 1}$ is monotone over $P$.
\end{lemma}

\begin{proof}
By~\Cref{claim:distance-invariant}, we have 
$$
\max_{(v, w) \in \viol_P(f_{\lceil \log h \rceil})} \dist(v, w) \leq \bigg \lceil \frac{h}{2^{\lceil \log h \rceil }} \bigg \rceil = 1
$$
Then $f_{\lceil \log h \rceil }$ has the property that all pairs that violate monotonicity are immediate neighbors in $P$. By one more application of \Cref{lemma: path shortening lemma}, we have 
\begin{align*}
&\max_{(v, w) \in \viol_P(f_{\lceil \log h \rceil + 1})} \dist(v, w) \\
&\leq \max\bigg (1 - 1, 1 - \bigg \lceil \frac{h}{2^{\lceil \log h \rceil + 1}} \bigg \rceil\bigg ) = 0,
\end{align*}
indicating that $f_{\lceil \log h \rceil + 1  }$ is monotone.
\end{proof}


%We will prove that the output $f_{\lceil \log h \rceil + 1}$ is close to $f_0$ via a special property of this algorithm, which is that it cannot increase the distance between $f_i$ and \emph{any} monotone function. This property is also a necessary component of the proof of \Cref{thm: the local corrector for general posets}. 
%
%\begin{lemma}[Error preservation]
%		\label{lem:error}
%For any $i$ and any monotone function $g$, $||f_i - q|| \le ||f_0 - q||$. 
%\end{lemma}
%\begin{proof}
%Let $f:~P \to \{0,1\}$ be a function and let $f'$ be obtained from $f$ by swapping the labels of two vertices $v, w$ such that $v \prec w$ and $f(v > f(w)$, and keeping all other labels the same. Since $g$ is monotone and $v$ and $w$ violate monotonicity in $f$, we must have one of the following cases: 
%\begin{itemize}
%	\item $f(v) \ne q(v)$ and $f(w) \ne q(w)$: Since $f(v) = 1$ and $f(w) = 0$, it must be the case that $g(v) = 0$ and $g(w) = 1$. Then making this swap decreases the error by $2/|P|$.
%	\item $f(v) \ne q(v)$ and $f(w) = q(w)$: Then $q(v)$ and $q(w)$ are both 0, and after the swap $f'(v) = q(v)$ and $f'(w) \ne q(w)$. The error does not change.
%	\item $f(v) = q(v)$ and $f(w) \ne q(w)$: This case is symmetrical to the last, and again the error does not change. 
%\end{itemize}
%The lemma follows by observing that each $f_i$ is obtained from $f_0$ by making a sequence of label swaps of violated pairs, and each swap cannot increase error with respect to $q$. 
%\end{proof}
%
%\begin{corollary}
%For any $f_i$, $||f_i - f_0||$ is at most twice the distance from $f_0$ to the closest monotone function. . 
%\end{corollary}
%
%\begin{proof}
%Let $q$ be the closest monotone function to $f_0$. Each swap cannot increase error with respect to $q$; therefore $||f_i - q|| \le ||f_0 - q||$, and so $||f_i - f_0|| \le 2||f_0 - q||$ by the triangle inequality.
%\end{proof}
%
\subsection{Local implementation}
\label{subsection: local implementation non-refined}
In this section, we provide an LCA that gives membership query access to the output of~\Cref{alg:global}, and we analyze its complexity. To better explain how our LCA simulates~\Cref{alg:global}, we present it as a system of three LCAs, each parameterized by the iteration number $i$. \Cref{alg:path graphs} makes queries to the $i_{th}$ function $f_i$ and an all-neighbors oracle for $P$, and answers queries to the $i_{th}$ $k$-violation graph $B_i$. \Cref{alg:matchings} makes queries to $B_i$ and answers queries to a maximal matching $\lambda_i$ over it. \Cref{alg:functions} makes queries to $f_i$ and $\lambda_i$ and answers queries to $f_{i+1}$, which swaps the matched labels.

%\begin{algorithm}[H]
%\begin{algorithmic}
%		\State Given: Target vertex $x$, directed all-neighbors query oracle $P$, membership query oracle $f_i$, height $h$.
%		\State Initialize $nbrs \gets \varnothing$, $k \gets \lceil h / 2^{i+1} \rceil $. 
%		\State Initialize $S$ to be the stack containing $(x, 0)$.
%		\While{$S$ is nonempty}
%		\State $(y, d) \gets pop(S)$
%		\If{$f_i(y) \ne f_i(x) \text{ and } d \ge k$} $nbrs \gets nbrs \cup \{y\}$
%		\EndIf
%		\If {$f_i(x) = 1$}
%			\For{$v \in P(y, out)$} $push(S, (v, d+1))$
%			\EndFor
%		\Else
%			\For{$v \in P(y, in)$} $push(S, (v, d+1))$
%			\EndFor
%		\EndIf
%		\EndWhile
%	\State \Return $nbrs$
%\end{algorithmic}
%\caption{An LCA for undirected all-neighbors queries $B_i(x, P, f_i, h, i)$ }
%\label{alg:path graphs}
%\end{algorithm}

\begin{algorithm}[H]
\begin{algorithmic}
		\State Given: Target vertex $x$, \red{all-neighbors (immediate predecessor and successor)} oracle for $P$, membership query oracle $f_i$, height $h$, iteration number $i$. 
		\State Initialize $k \gets \lceil h / 2^{i+1} \rceil$
		\If {$f_i(x) = 1$}
		\State $S \gets$ the set of all successors of $x$ %\blue{Arsen:
		%distance is max-distance, we should make sure this creates no trouble for non-graded posets.}
		\Else
		\State $S \gets$ the set of all predecessors of $x$ 
		\EndIf
		\State Compute longest path $\dist(x, y)$ for each $y \in S$ by dynamic programming
		\State Remove any $y$ from $S$ such that $\dist(x, y) < k$ or $f(y) = f(x)$
		\State \Return $S$
		
\end{algorithmic}
\caption{An LCA for undirected all-neighbors queries $B_i(x, P, f_i, h, i)$ }
\label{alg:path graphs}
\end{algorithm}

\begin{algorithm}[H]
\begin{algorithmic}
		\State Given: Target vertex $x$, undirected all-neighbors query oracle $B_i$, random seed $r$, and confidence parameter $\delta$.
		\State Call the algorithm described in \Cref{cor:matchings} with $B_i$ as the graph, $x$ as the target, and $r$ as the random seed \blue{ and $\Delta$ as the degree bound}. If $x$ is in the matching, return the vertex that it is matched to; otherwise return $x$.
\end{algorithmic}
\caption{An LCA for maximal matchings $\lambda_i(x, B_i, r, \delta)$}
\label{alg:matchings}
\end{algorithm}

\begin{algorithm}[H]
\begin{algorithmic}
		\State Given: Target vertex $x$, matching query oracle $\lambda_i$, membership query oracle $f_{i}$
		\State \Return $f_{i}(\lambda_i(x))$
\end{algorithmic}
\caption{An LCA for membership queries $f_{i+1}(x, \lambda_i, f_i)$}
\label{alg:functions}
\end{algorithm}

\subsubsection{Analysis of our implementation}
\label{subsubsection: analysis of our implementation}
Throughout this section, for any algorithm $A$, the notation $T(A)$ denotes the running time of $A$. 

\begin{claim}[Behavior of $B_i$]
\label{claim:gi-behavior}
For any $0 \le i \le \lceil \log h \rceil + 1$, $B_i$ provides all-neighbors query access to the $\lceil h/2^{i+1}\rceil$-violation graph of $P$ with respect to $f_i$. Furthermore, if each element of $P$ has at most $\Delta$ successors or predecessors, then $T(B_i) \le O(\Delta \cdot T(f_i))$.
\end{claim}
\begin{proof}
If $f_i(x) = 1$, then all neighbors of $x$ in the $\lceil h/2^{i+1}\rceil$-violation graph of $P$ are successors of $x$. Finding all the successors takes $O(\Delta)$ time by depth-first search. Computing $\dist(x, y)$ for each successor $y$ of $x$ takes $O(\Delta)$ time by standard dynamic programming techniques for finding longest paths in a DAG. Comparing $f_i(x)$ to $f_i(y)$ takes $O(\Delta)$ queries to $f_i$, and therefore $O(\Delta \cdot T(f_i))$ time. The case of $f_i(x) = 0$ is symmetric.
\end{proof}
%\gray{
%\begin{proof}
%It suffices to show that for any target vertex $x$, the return set $nbrs$ contains all vertices at distance at least $\lceil h/2^{i+1} \rceil$ from $x$ that violate monotonicity with respect to $f_i$ and $x$. Note that $B_i$ performs a DFS of $P$ in one direction (outgoing edges if $f_i(x) = 1$, incoming edges if $f_i(x) = 0$) while tracking the distance from $x$. All vertices that violate monotonicity with respect to $x$ must lie in this direction, so the DFS will explore them all. These vertices are exactly those whose function value differs from $f_i(x)$. Vertices are added to $nbrs$ if the function value differs from $f_i(x)$ and there exists a path from $x$ of length at least $\lceil h / 2^{i+1} \rceil$, as desired. \\
%
%The DFS explores only vertices that have a directed path from $x$ in $P$, so the number of vertices explored cannot exceed $\Delta$. $B_i$ makes one membership query to $f_i$ for each vertex explored, yielding the running time of $\Delta \cdot T(f_i)$.
%\end{proof}
%}
\begin{claim}[Behavior of $\lambda_i$]
\label{claim:li-behavior}
For any $0 \le i \le \lceil \log h \rceil + 1$, and $\delta \in (0,1]$, $\lambda_i$ provides query access to a maximal matching over $B_i$ with probability $1 - \delta/(\lceil \log h \rceil + 1)$, using a random seed of length $\red{\poly(\Delta\log(N/\delta))}$. Furthermore, $T(\lambda_i) \le \red{\poly(\Delta \log(N/\delta)) \cdot T(B_i)}$.
\end{claim}
\begin{proof}
Let $\delta' = \delta/(\lceil \log h \rceil + 1)$.
By \Cref{cor:matchings}, $\lambda_i$ fails with probability at most $\delta'$, where the query complexity and the length of the random seed are each $\red{\poly(\Delta \log(N/\delta'))}$. Since $h$ is always at most $\Delta$, this is still $\red{\poly(\Delta\log(N/\delta))}$.
The claim follows from the fact that since the queries are made to $B_i$, each query takes time $T(B_i)$. 
\end{proof}
We now proceed with our proof of \Cref{thm: the local corrector for general posets}, which we restate here for convenience.
\main*

\begin{proof} 
Assume that for each $i \le \lceil \log h \rceil + 1$, the matching provided by $\lambda_i$ is maximal for $B_i$. Under this condition, $f_i$, $\lambda_i$, and $B_i$ implement LCAs for all the objects expected by \Cref{alg:global} (by \Cref{claim:gi-behavior} and \Cref{claim:li-behavior}). The correctness result of \Cref{lem:correctness} implies that our implementation of $f_{\lceil \log h \rceil + 1}$ is an LCA for a function with the properties claimed in this theorem. We will bound the running time and query complexity by a recurrence relation.
		
As a base case, we will let $T(f_0)$ be 1. We have three recurrences: $T(B_i) \le O(\red{\Delta} \cdot T(f_i))$, $T(\lambda_i) \le \red{\poly(\Delta \log(N/\delta))} \cdot T(B_i)$, and $T(f_{i+1}) \le O(T(f_i) + T(\lambda_i))$. To simplify: \\
\begin{align*} 
T(f_{i+1}) &\le O(T(f_i) + T(\lambda_i)) \\
		   &\le T(f_i) + \red{\poly(\Delta \log(N/\delta))} \cdot T(B_i) \\
		   &\le T(f_i) + \red{\poly(\Delta \log(N/\delta)) \cdot \Delta} T(f_i) \\
		   &\le \red{\poly(\Delta \log(N/\delta))} \cdot T(f_i) \\
\end{align*}
This recurrence resolves to 
\[T(f_i) = \red{(\Delta \log(N/\delta))^{O(i)}}\]
for both running time and query complexity. Letting $i = \lceil \log h \rceil + 1$, we have a total running time and query complexity of $\red{(\Delta \log(N/\delta))^{O(\log h)}}$. 

We initialize our algorithm with a random bit string of length $\red{\poly(\Delta \log (N/\delta))}$ as required by \Cref{claim:li-behavior}. Each call to $\lambda_i$ fails with probability $\delta/(\lceil \log h \rceil + 1)$; this gives a total failure probability of $\delta$. Therefore, with probability at least $1 - \delta$ all the matchings are maximal and our analysis holds.
\end{proof}




==> Monotone corrector new arxiv version/intro.tex <==
\input{abstract}
\section{Introduction}
%\subsection{Main result: proper learning of monotone functions.}

\paragraph{Proper learning of monotone functions.} Consider the \emph{proper learning} problem for monotone functions:
\begin{center}
\textit{
Given i.i.d uniform labeled examples from an unknown monotone $g:\{0,1\}^n\rightarrow \{0,1\}$, output a predictor computing monotone $\hat{g}:\{0,1\}^n\rightarrow \{0,1\}$ that predicts $g$ correctly on at least $1-\epsilon$ fraction of the domain. 
}
\end{center}
For over 25 years there has been a large statistical-to-computational gap in our understanding of this problem. 
A $2^{\tilde{O}(\sqrt{n}/\eps)}$-time \emph{improper} learning algorithm --- that is, an algorithm that outputs a predictor $f$ that is accurate but not guaranteed to be monotone --- is given in \cite{bshouty1996fourier}.
%\gray{Specifically, the work of \cite{bshouty1996fourier} gives a $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$-time algorithm for obtaining a predictor $f$ that itself is not guaranteed to be monotone (such learner is called \textbf{improper}).}
One could use the output of this algorithm to 
obtain a monotone $\hat{g}$ by computing $f$ on every element of $\{0,1\}^n$ and solving a linear program to obtain the closest monotone function to $f$. Although this gives a $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$-sample algorithm, the run-time is $2^{\Omega(n)}$. No proper learning algorithm with faster run-time was known.

Through a new connection with local computation algorithms, we close this gap by giving a $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$-time algorithm for this problem. Note that the running time essentially matches that of the aforementioned improper learning algorithm of \cite{bshouty1996fourier}. Moreover, our algorithm is essentially optimal, due to the $2^{\Tilde{\Omega}(\sqrt{n})}$ query lower bound of \cite{blais2015learning}. 
Furthermore, our algorithm is robust to adversarial noise in the labels. Specifically, in the agnostic learning model of Kearns, Schapire, and Sellie \cite{kearns1994toward}, our algorithm can handle a noise rate of $\Omega(\epsilon)$.     

\paragraph{Monotonicity testing.}
The question of testing monotonicity of an unknown Boolean function over $\{0,1\}^n$ (given query access) has received a large amount of attention  
\cite{goldreich_testing_1998,chakrabarty_on_2013,chen_new_2014,chen_boolean_2015,khot_monotonicity_2015,belovs_polynomial_2016,chen_beyond_2017}. However, the algorithms in this line of work possess the drawback of having a large \emph{tolerance ratio}\footnote{A tester for monotonicity distinguishes a monotone function from a function that is $\epsilon$-far from monotone.
In this work, we use tolerance ratio $\alpha$ to  mean that the tester will accept a function $\epsilon/\alpha$-close to monotone.}, i.e. they will reject some functions that are extremely close to monotone. The more recent work of \cite{pallavoor2022approximating} gives a tester with tolerance ratio of $\tilde{O}(\sqrt{n})$, and this is the best tolerance ratio known\footnote{Note that Theorem 1.8 of \cite{CanonneGG0W16} gives a $2^{o(n)}$-query algorithm (no run-time bound is claimed). The run-time is still $2^{\Omega(n)}$ due to step 8 of their Algorithm 2 on page 31.} for a $2^{o(n)}$-run-time algorithm.  

As a simple corollary of our proper learning algorithm,
one can already achieve \emph{constant tolerance ratio for monotonicity testing with  $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$ run-time} via a well-known connection between learning and testing \cite{goldreich1998property}. (We emphasize that, to draw this corollary, it is critical that the learning algorithm is proper and robust to noise in labels.) Further, building more directly on our technical ideas, we present a constant-tolerance monotonicity tester with \emph{exponentially better dependence on $\epsilon$ of $2^{\Tilde{O}\left(\sqrt{n \log \frac{1}{\epsilon}}  \right)}$}. This approach also yields a tolerant tester for functions over general posets, which we describe in detail in \textbf{todo: link section}. 

%The work of \cite{} builds upon this line of work to give an algorithm of tolerance ratio of $\tilde{O}(\sqrt{n})$
%are not guaranteed to be \textbf{tolerant}\footnote{A regular tester for monotonicity distinguishes between monotone functions and functions $\epsilon$-far from monotone. A \textbf{tolerant} tester for monotonicity for some absolute constant $C$ distinguishes functions that are $\epsilon/C$-close to monotone from functions $\epsilon$-far from monotone.}. In fact, these algorithms could reject functions as close as $\frac{\epsilon}{\poly(n)}$ to monotone.
%Through a well-known connection between learning and testing \cite{goldreich1998property}, as a corollary of our result we obtain a $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$-time \textbf{tolerant tester for monotonicity} of an unknown function $g:\{0,1\}^n\rightarrow \{0,1\}$. In other words, for some absolute constant $C$, in time $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$ we can test if $g$ is $\frac{\epsilon}{C}$-close to monotone or $\epsilon$-far from monotone. Here also,
%no algorithm with non-trivial run-time was known previously. We emphasize that to draw this corollary it is critical that the learning algorithm is proper (robustness to noise in labels is also important).  


%Over the years, the study of monotone Boolean functions over the Boolean cube has been an important direction in our field. 
%\textbf{todo: cite O'Donnell book?} 



\subsection{Monotonicity correction via sorting on partially ordered sets.}
%\textbf{todo: list of cites on local correction} Our core idea is a {\sl local corrector} for monotonicity: an algorithm that takes some input $x$, makes queries to a black-box function $f$, and outputs $f_{mon}(x)$ where $f_{mon}$ is a monotone function that is close to $f$ in Hamming distance, if such a function exists. A local corrector, combined with any improper hypothesis, yields a proper hypothesis (similarly, a local corrector combined with a Hamming-distance test yields a tolerant test for monotonicity). The efficiency of the local corrector determines how quickly the proper hypothesis can be evaluated. The running time of our corrector is polynomial in the number of coefficients in the hypothesis of \cite{bshouty1996fourier}, the state-of-the-art improper learner for monotone functions. This allows their hypothesis to be made proper with a polynomial increase in its evaluation time. \\

\paragraph{Parallelizing greedy algorithms.} One of our core ideas is to bridge our learning task with a large body of work on \emph{parallelizing greedy algorithms}. [citations] 
Greedy algorithms are often useful for outputting one of many possible labelings on a large domain --- for example the indicator of a maximal independent set on a large graph. 
Such algorithms work as follows: choose some ordering on the vertices, and fix the label on each one conditioned on the labels of vertices that come earlier in the ordering. 
In a distributed setting, the goal is for each vertex to output its own label without needing to simulate all the vertices that come before it in the ordering. 
We call this ``parallelizing'' a greedy algorithm. 
We present a problem of this type for which a greedy algorithm is known, and a ``parallelized'' greedy algorithm would yield an efficient proper learner for monotone functions. 

\paragraph{The poset-sorting problem.} One of our core ideas is to bridge our learning task with a large body of work on parallelizing greedy algorithms in the setting of local and distributed computing. There exists a large body of work on this topic: see [] for an overview. (\cite{Ghaffari16} add references talk about MIS).
Specifically, we introduce the problem of {\em poset sorting}, that is, sorting binary values on a partially ordered set (poset), which we believe is of independent interest: 
\begin{center}
\textit{
Let $P$ be poset of $N$ elements with longest chain length at most $h$ and such that every element has at most $\Delta$ predecessors or successors. Given a binary labeling $f$ of elements of $P$, output a new binary labeling $f_\text{mon}$ that (i) is monotone with respect to the partial order in $P$ (ii) can be obtained from $f$ by a sequence of swaps of monotonicity-violating label pairs. 
}
\end{center}

Why is an algorithm for sorting on a poset $P$ relevant to proper learning? Suppose we obtained an improper predictor $f$ via the algorithm of \cite{bshouty1996fourier}, in the form of a circuit computing $f$. Then, let monotone $f_\text{mon}$ be obtained from $f$ by flipping a sequence of monotonicity-violating labels. It is not hard to argue that since $f$ was $O(\epsilon)$-close to the monotone $g$ we are trying to learn, then so is $f_\text{mon}$. Therefore, if we manage to transform the small circuit computing $f$ into a small circuit computing such $f_\text{mon}$, then proper learning is accomplished. 
What guarantee does one need from the sorting algorithm to accomplish such transformation? Roughly, one needs that to evaluate $f_\text{mon}$ at a given element $x$ the algorithm needs to compute $f$ on only a small number of points (and have an appropriately fast run-time). If we have a sorting algorithm satisfying this guarantee, then we can augment the circuit for $f$ with a circuit that executes this sorting algorithm, and as a result obtain a small circuit for $f_\text{mon}$. It turns out that problems about this exact type of guarantee have been studied in the so-called LCA (local computation algorithm) model. 

\paragraph{How we obtain an LCA for poset sorting problem.} 

Furthermore, it has been studied extensively how to implement various greedy algorithms in this model\footnote{This turns out to be intimately connected to implementing greedy algorithms in the distributed local model and in the massively parallel computation model}.     

\emph{parallelizing greedy algorithms}. [citations] 
Greedy algorithms are often useful for outputting one of many possible labelings on a large domain --- for example the indicator of a maximal independent set on a large graph. 
Such algorithms work as follows: choose some ordering on the vertices, and fix the label on each one conditioned on the labels of vertices that come earlier in the ordering. 
In a distributed setting, the goal is for each vertex to output its own label without needing to simulate all the vertices that come before it in the ordering. 
We call this ``parallelizing'' a greedy algorithm. 
We present a problem of this type for which a greedy algorithm is known, and a ``parallelized'' greedy algorithm would yield an efficient proper learner for monotone functions. 

An eye-catching property of the poset problem 



%Fortunately, algorithms satisfying this exact type of guarantee that is provided by the LCA (local computation algorithm) model.  


There is 


%A small circuit for the sorting problem then allows one to obtain a small circuit for such $f_\text{mon}$, without having to write out the whole function. This allows one to use $f_\text{mon}$ as a proper hypothesis. 



Thus, to accomplish our task we need an 

Clearly, there is a greedy algorithm for sorting that swaps monotonicity-violating pairs of labels until there are none left.
The challenge is to do this in a local fashion; i.e., to output the sorted label for a vertex without computing the entire sorted labeling.
Among the many distributed and parallel computation models, the one that is most relevant to us is the {\sl local computation algorithm} (LCA) model, defined formally in \cite{RTVX11, AlonRVX12}.
LCAs are well-studied in the literature on distributed and sublinear algorithms (some examples include
\cite{RTVX11, AlonRVX12,levi_local_2015, Ghaffari16,
reingold_new_2014, even_best_2014, ChangFGUZ19}).
In brief, to be an LCA, an algorithm should be local in the sense that it should not need to read the entire assignment of labels to vertices in order to determine which label will end up at some particular vertex $\vect{x}$. It should suffice to read only the labels of vertices that lie in a restricted neighborhood of $\vect{x}$ --- ideally not much more than the set of vertices one would need to read in order to determine whether $\vect{x}$'s own label violates monotonicity. We explain the algorithm itself in Subsection \ref{subsection: the algorithm summary}. \\

%As a result, the running time and query complexity of this algorithm depend primarily on $\Delta$ and $h$. 
%Specifically, in the LCA model of distributed computation, given query access to $P$ and $f$ we need to implement query access to  $f_\text{mon}$. 


\paragraph{Proper learning via local correction.} Why is an LCA for sorting on a poset $P$ relevant to proper learning? Suppose we obtained an improper predictor $f$ via the algorithm of \cite{bshouty1996fourier}. Then, let monotone $f_\text{mon}$ be obtained from $f$ by flipping a sequence of monotonicity-violating labels. It is not hard to argue that since $f$ was $O(\epsilon)$-close to the monotone $g$ we are trying to learn, then so is $f_\text{mon}$. An LCA then allows one to obtain a fast evaluator for such $f_\text{mon}$, without having to write out the whole function. This allows one to use $f_\text{mon}$ as a proper hypothesis. 
%\gray{Furthermore, this LCA allows one to obtain a tolerant tester for functions over general posets, rather than just the Boolean cube.}

In other words, an LCA for sorting on a poset is a {\sl local corrector} for monotonicity: an algorithm that takes some input $x$, makes queries to a black-box function $f$, and outputs $f_{mon}(x)$ where $f_{mon}$ is a monotone function that is close to $f$ in Hamming distance, if such a function exists. Local correctors for various function properties are studied in \cite{ACCL07, SS10} \textbf{todo: more cites on local correction}. A local corrector, combined with any improper hypothesis, yields a proper hypothesis. The efficiency of the LCA determines how quickly the proper hypothesis can be evaluated.

\paragraph{Tolerant monotonicity testing via local correction.}...\\


Stepping back, we give an application of LCAs to the setting of (centralized) PAC learning and tolerant testing --- a connection that is less discussed but we believe is quite natural. Efficient local correctors may exist for many function classes, and this connection may yield more algorithms for both learning and testing.


\subsection{Our LCA for sorting on a poset.}\label{subsection: the algorithm summary}

When the longest chain length $h$ is 1, this problem is equivalent to the classical problem of finding a maximal matching on a bipartite graph with $N$ vertices and maximum degree at most $\Delta$. We note that a recent LCA by Ghaffari and Uitto 
\cite{GhaffariU19} handles this problem using a run-time of $\Delta^{O(\log\log \Delta)}\polylog(N)$. \red{ Maybe emphasize here that Ghaffari and Uitto is a powerful result that followed a long line of research?}



For larger values of $h$, a naive approach would be to execute a sequence of phases, in each of which a maximal matching between monotonicity-violating labels is produced and the labels that are matched with each other are swapped. One can show that $O(h)$ such phases suffice and sometimes necessary if the matchings are arbitrary. If the algorithm of \cite{GhaffariU19} is used to implement each of the phases, this yields a run-time of $\left(\Delta^{O(\log\log \Delta)}\polylog(N)\right)^h$.
For properly learning monotone functions over the Boolean cube, the parameters\footnote{These are the parameters for small constant $\epsilon$. A slight subtlety in our argument is that we need to work over truncated hypercube, i.e. handle separately $O(\epsilon)$ fraction of the elements with too high or too low Hamming weight. This is a standard technique, and in our case it makes the parameter $\Delta$ in our poset small enough for us to get a good run-time guarantee using our poset sorting algorithm.
} we are primarily interested in are $h =\Theta(\sqrt{n})$, $\Delta = 2^{\tilde{\Theta}(\sqrt{n})}$ and $N=\Theta(2^n)$.
The naive approach then gives us a run-time of $\left(\Delta^{O(\log\log \Delta)} \polylog(N)\right)^h=2^{\Omega(n)}$, which is too slow for our purposes.

We beat the naive approach by enforcing that the maximal matchings at each step only include pairs of vertices that are sufficiently far away in the graph.
We show that after each matching step, the greatest distance between pairs that violate monotonicity reduces by a factor of 2. This allows us to reduce the exponent from $h$ to $\log h$, which is sufficiently fast to yield an essentially optimal proper learner for monotone functions. \\


%\gray{Our local corrector must sort labels in a truncated region of the Boolean cube, which is a poset of height $h = \tilde{O}(\sqrt{n})$ and $\Delta = 2^{\tilde{O}(\sqrt{n})}$. To give local access to the sorted configuration of labels in $2^{o(n)}$ time, we require a more general algorithm that scales well with $h$. To achieve an exponent of $\log h$ rather than $h$, we enforce that the maximal matchings at each step only include pairs of vertices that are sufficiently far away in the graph.} \\  

%How does such an algorithm help with proper learning of monotonicity? We may truncate the Boolean cube to only the vertices of Hamming weight $n/2 \pm \tilde{O}(\sqrt{n})$ and sort the labels in this truncated region. The sorting works by matching pairs of vertices that are sufficiently far from each other and whose labels violate monotonicity, and swapping them. We harness an efficient LCA for finding maximal matchings \cite{GhaffariU19}, which comes from a long line of work on parallelizing greedy graph algorithms [\textbf{todo: list of cites}]. The argument goes roughly as follows.  \\

%\gray{We show that the process of swapping labels between pairs that violate monotonicity cannot increase the Hamming distance between the function and any monotone function, and therefore cannot increase the error beyond the distance to monotonicity.} \\

\subsection{Other related work}
\textbf{todo: jane}
The problem of locally correcting monotonicity has been studied in \cite{ACCL07} and \cite{SS10}, in various parameter settings. The work of \cite{ACCL07} introduces the problem of online property reconstruction and gives an algorithm for this task for real-valued functions over the discrete numberline $[n]$. The work of \cite{SS10} introduces the framework of local property reconstruction, which is the same framework our approach uses (i.e., local correction by parallelizable LCA). They give a local corrector for functions over the hypergrid $[n]^d$, with large dependence on $d$ but small dependence on $n$.\\ 

Lower bounds: \cite{BGJ+10},
Parnas Ron Rubinfeld (introduced tolerant testing): \cite{Parnas2004TolerantPT},








==> Monotone corrector new arxiv version/intro2.tex <==
%\input{abstract}
\section{Introduction}
%\subsection{Main result: proper learning of monotone functions.}

\textbf{Proper learning of monotone functions.} Consider the \emph{proper learning} problem for monotone functions:
\begin{center}
\textit{
Given i.i.d uniform labeled examples from an unknown monotone $g:\{0,1\}^n\rightarrow \{0,1\}$, output a monotone, $\eps$-accurate predictor $\hat{g}:\{0,1\}^n\rightarrow \{0,1\}$ --- that is, a circuit computing a monotone function that agrees with $g$ on at least $1-\epsilon$ fraction of the domain. 
}
\end{center}
For over 25 years there has been a large statistical-to-computational gap in our understanding of this problem. 
A $2^{\tilde{O}(\sqrt{n}/\eps)}$-time \emph{improper} learning algorithm --- that is, an algorithm that outputs a predictor $f$ that is accurate but not guaranteed to be monotone --- is given in \cite{bshouty1996fourier}.
%\gray{Specifically, the work of \cite{bshouty1996fourier} gives a $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$-time algorithm for obtaining a predictor $f$ that itself is not guaranteed to be monotone (such learner is called \textbf{improper}).}
One could use the output of this algorithm to 
obtain a monotone $\hat{g}$ by computing $f$ on every element of $\{0,1\}^n$ and solving a linear program to obtain the closest monotone function to $f$. Although this gives a $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$-sample algorithm, the run-time is $2^{\Omega(n)}$. No proper learning algorithm with faster run-time (i.e. $2^{o(n)}$) was known, even given query access to $g$.

Through a new connection with local computation algorithms, we close this gap by giving a $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$-time algorithm for this problem. Note that the running time essentially matches that of the aforementioned improper learning algorithm of \cite{bshouty1996fourier}. Moreover, our algorithm is essentially optimal, due to the $2^{\Tilde{\Omega}(\sqrt{n})}$ query lower bound of \cite{blais2015learning}. 
Furthermore, our algorithm is robust to adversarial noise in the labels. Specifically, in the agnostic learning model of Kearns, Schapire, and Sellie \cite{kearns1994toward}, our algorithm can handle a noise rate of $\Omega(\epsilon)$.     

\textbf{Monotonicity testing.}
The question of testing monotonicity of an unknown Boolean function over $\{0,1\}^n$ (given query access) has received a large amount of attention  
\cite{goldreich_testing_1998, DodisGLRRS99,chakrabarty_on_2013,chen_new_2014,chen_boolean_2015,khot_monotonicity_2015,belovs_polynomial_2016,chen_beyond_2017}. However, the algorithms in this line of work possess the drawback of having a large \emph{tolerance ratio}\footnote{A tester for monotonicity distinguishes a monotone function from a function that is $\epsilon$-far from monotone.
In this work, we use tolerance ratio $\alpha$ to  mean that the tester will accept a function $\epsilon/\alpha$-close to monotone.}, i.e. they will reject some functions that are extremely close to monotone. The more recent work of \cite{pallavoor2022approximating} gives a tester with tolerance ratio of $\tilde{O}(\sqrt{n})$, and this is the best tolerance ratio known\footnote{Note that Theorem 1.8 of \cite{CanonneGG0W16} gives a $2^{o(n)}$-query algorithm (no run-time bound is claimed). The run-time is still $2^{\Omega(n)}$ due to step 8 of their Algorithm 2 on page 31.} for a $2^{o(n)}$-run-time algorithm.  

As a simple corollary of our proper learning algorithm,
one can already achieve \emph{constant} tolerance ratio for monotonicity testing with  $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$ run-time via a well-known connection between learning and testing \cite{goldreich1998property}. (We emphasize that, to draw this corollary, it is critical that the learning algorithm is proper and robust to noise in labels.) Even more, building more directly on our technical ideas, we present a constant-tolerance monotonicity tester with \emph{exponentially better dependence on $\epsilon$ of $2^{\Tilde{O}\left(\sqrt{n \log \frac{1}{\epsilon}}  \right)}$}. This approach also yields a tolerant monotonicity tester for functions over general posets, which we describe in detail in \Cref{cor:poset tester}. By a standard reduction \cite{Parnas2004TolerantPT}, this also gives an approximator for distance to monotonicity (within a constant multiplicative error plus an $\eps N$ additive error) in functions over general posets as well.

%The work of \cite{} builds upon this line of work to give an algorithm of tolerance ratio of $\tilde{O}(\sqrt{n})$
%are not guaranteed to be \textbf{tolerant}\footnote{A regular tester for monotonicity distinguishes between monotone functions and functions $\epsilon$-far from monotone. A \textbf{tolerant} tester for monotonicity for some absolute constant $C$ distinguishes functions that are $\epsilon/C$-close to monotone from functions $\epsilon$-far from monotone.}. In fact, these algorithms could reject functions as close as $\frac{\epsilon}{\poly(n)}$ to monotone.
%Through a well-known connection between learning and testing \cite{goldreich1998property}, as a corollary of our result we obtain a $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$-time \textbf{tolerant tester for monotonicity} of an unknown function $g:\{0,1\}^n\rightarrow \{0,1\}$. In other words, for some absolute constant $C$, in time $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$ we can test if $g$ is $\frac{\epsilon}{C}$-close to monotone or $\epsilon$-far from monotone. Here also,
%no algorithm with non-trivial run-time was known previously. We emphasize that to draw this corollary it is critical that the learning algorithm is proper (robustness to noise in labels is also important).  


%Over the years, the study of monotone Boolean functions over the Boolean cube has been an important direction in our field. 
%\textbf{todo: cite O'Donnell book?} 



\subsection{Monotonicity correction via sorting on partially ordered sets.}
%\textbf{todo: list of cites on local correction} Our core idea is a {\sl local corrector} for monotonicity: an algorithm that takes some input $x$, makes queries to a black-box function $f$, and outputs $f_{mon}(x)$ where $f_{mon}$ is a monotone function that is close to $f$ in Hamming distance, if such a function exists. A local corrector, combined with any improper hypothesis, yields a proper hypothesis (similarly, a local corrector combined with a Hamming-distance test yields a tolerant test for monotonicity). The efficiency of the local corrector determines how quickly the proper hypothesis can be evaluated. The running time of our corrector is polynomial in the number of coefficients in the hypothesis of \cite{bshouty1996fourier}, the state-of-the-art improper learner for monotone functions. This allows their hypothesis to be made proper with a polynomial increase in its evaluation time. \\



\textbf{The poset-sorting problem.} One of our core ideas is to create a new bridge between our learning task and recent exciting developments on parallelizing greedy algorithms \cite{Ghaffari16, GhaffariU19, Ghaffari22}. These developments accomplish speedups for classic graph problems in the setting of local and distributed computing. They build on a large body of work in local computation algorithms and distributed graph algorithms: some examples include
\cite{RTVX11, AlonRVX12, levi_local_2015, GoosHLMS15, 
reingold_new_2014, even_best_2014, ChangFGUZ19, EvenLMR21, ParterRVY19, ArvivL21, BrandtGR21, GrebikR21}.
In order to accomplish this, we introduce the problem of poset sorting, that is, sorting binary values on a partially ordered set (poset), which we believe is of independent interest: 
\begin{center}
\textit{
Let $P$ be a poset of $N$ elements with longest chain length at most $h$ and such that every element has at most $\Delta$ predecessors or successors. Given a binary labeling $f$ of elements of $P$, output a new binary labeling $f_\text{mon}$ that (i) is monotone with respect to the partial order in $P$ (ii) can be obtained from $f$ by a sequence of swaps of monotonicity-violating label pairs. 
}
\end{center}
Clearly, there is a greedy algorithm for this task that keeps swapping monotonicity-violating pairs of labels until there are none left. 
The challenge is to do this in a distributed fashion.
Among the many distributed and local computation models, the one that turns out relevant to us is the {\sl local computation algorithm} (LCA) model, defined formally in \Cref{sec:prelim}.
%LCAs are well-studied in the literature on distributed and sublinear algorithms (some examples include
%\cite{RTVX11, AlonRVX12, levi_local_2015, Ghaffari16, %reingold_new_2014, even_best_2014, ChangFGUZ19}).
In brief, to be an LCA, an algorithm should be local in the sense that it should not need to read the entire assignment of labels to vertices in order to determine which label will end up at some particular vertex $x$. It should suffice to read only the labels of vertices that lie in a restricted neighborhood of $x$ --- ideally not much more than the set of vertices one would need to read in order to determine whether $x$'s own label violates monotonicity. We explain the algorithm itself in Subsection \ref{subsection: the algorithm summary}. 
%As a result, the running time and query complexity of this algorithm depend primarily on $\Delta$ and $h$. 
%Specifically, in the LCA model of distributed computation, given query access to $P$ and $f$ we need to implement query access to  $f_\text{mon}$. 

\textbf{Proper learning via local correction.} 
Why is an algorithm for sorting on a poset $P$ relevant to proper learning? Suppose we obtained an improper predictor $f$ via the algorithm of \cite{bshouty1996fourier}, in the form of a small circuit computing $f$. Then, let monotone $f_\text{mon}$ be obtained from $f$ by flipping a sequence of monotonicity-violating labels.
It is not hard to argue that since $f$ is $O(\epsilon)$-close to the monotone $g$ we are trying to learn, then so is any $f_\text{mon}$ obtained in this manner (see \Cref{remark: sorting implies local correction} for more details). What the LCA allows us to do is to transform the circuit computing $f$ into a \emph{small} circuit computing such $f_\text{mon}$. 
The reason is that to evaluate $f_\text{mon}$ at a given element $x$ the LCA evaluates $f$ on only a small number of points and has an appropriately fast run-time. This allows us to augment the circuit for $f$ with a circuit that executes this sorting algorithm, and as a result obtain a small circuit for $f_\text{mon}$. 


In other words, an LCA for sorting on a poset is a {\sl local corrector} for monotonicity: an algorithm that takes some input $x$, makes queries to a black-box function $f$, and outputs $f_{mon}(x)$ where $f_{mon}$ is a monotone function that is close to $f$ in Hamming distance, if such a function exists. 
Examples of local correctors for various function properties
can be found in 
\cite{AilonCCL08,  ACCL07, SS10, KalePS08,  CampagnaGR13, JhaR13, AJMR14, Comandur16}. A local corrector, combined with any improper hypothesis, yields a proper hypothesis. The efficiency of the LCA determines how quickly the proper hypothesis can be evaluated.

%\paragraph{Tolerant monotonicity testing via local correction.}...\\


%Stepping back, we give an application of LCAs to the setting of (centralized) PAC learning and tolerant testing --- a connection that is less discussed but we believe is quite natural. Efficient local correctors may exist for many function classes, and this connection may yield more algorithms for both learning and testing.

\subsection{Our LCA for sorting on a poset.}\label{subsection: the algorithm summary}

When the longest chain length $h$ is 1, then the poset-sorting problem is equivalent to the classical problem of finding a maximal matching on a bipartite graph with $N$ vertices and maximum degree at most $\Delta$. We note that a recent LCA by Ghaffari \blue{\cite{Ghaffari22}} handles this problem using a run-time of only \blue{$
\poly(\Delta, \log(N/\delta))$}. 

For larger values of $h$, a naive approach would be to execute a sequence of phases, in each of which a maximal matching between monotonicity-violating labels is produced and the labels that are matched with each other are swapped. One can show that $O(h)$ such phases suffice and sometimes necessary if the matchings are arbitrary. If the algorithm by Ghaffari \cite{Ghaffari22} is used to implement each of the phases, this yields a run-time of $\left(\blue{
\Delta \log(N/\delta)} \right)^{\Theta(h)}$.
For properly learning monotone functions over the Boolean cube, the parameters\footnote{These are the parameters for small constant $\epsilon$. A slight subtlety in our argument is that we need to work over truncated hypercube, i.e. handle separately $O(\epsilon)$ fraction of the elements with too high or too low Hamming weight. This is a standard technique, and in our case it makes the parameter $\Delta$ in our poset small enough for us to get a good run-time guarantee using our poset sorting algorithm.
} we are primarily interested in are $h =\Theta(\sqrt{n})$, $\Delta = 2^{\tilde{\Theta}(\sqrt{n})}$ and $N=\Theta(2^n)$.
The naive approach then gives us a run-time of $\left(\blue{
\Delta \log(N/\delta)} \right)^{\Theta(h)}=2^{\Omega(n)}$, which is too slow for our purposes.

We beat the naive approach by enforcing that the maximal matchings at each step only include pairs of vertices that are sufficiently far away in the graph.
We show that after each matching step, the greatest distance between pairs that violate monotonicity reduces by a factor of 2. This allows us to reduce the exponent from $h$ to $\log h$, which is sufficiently fast to yield an essentially optimal proper learning algorithm for monotone functions. 


%\gray{Our local corrector must sort labels in a truncated region of the Boolean cube, which is a poset of height $h = \tilde{O}(\sqrt{n})$ and $\Delta = 2^{\tilde{O}(\sqrt{n})}$. To give local access to the sorted configuration of labels in $2^{o(n)}$ time, we require a more general algorithm that scales well with $h$. To achieve an exponent of $\log h$ rather than $h$, we enforce that the maximal matchings at each step only include pairs of vertices that are sufficiently far away in the graph.} \\  

%How does such an algorithm help with proper learning of monotonicity? We may truncate the Boolean cube to only the vertices of Hamming weight $n/2 \pm \tilde{O}(\sqrt{n})$ and sort the labels in this truncated region. The sorting works by matching pairs of vertices that are sufficiently far from each other and whose labels violate monotonicity, and swapping them. We harness an efficient LCA for finding maximal matchings \cite{GhaffariU19}, which comes from a long line of work on parallelizing greedy graph algorithms [\textbf{todo: list of cites}]. The argument goes roughly as follows.  \\

%\gray{We show that the process of swapping labels between pairs that violate monotonicity cannot increase the Hamming distance between the function and any monotone function, and therefore cannot increase the error beyond the distance to monotonicity.} \\

\subsection{Other related work}
The problem of locally correcting monotonicity has been studied in \cite{AilonCCL08,ACCL07, SS10, BGJ+10, AJMR14} 
in various parameter settings. 
The work of \cite{AilonCCL08} introduces the problem of online property reconstruction and gives an algorithm for correcting monotonicity for real-valued functions over the discrete number line. The work of \cite{Parnas2004TolerantPT} gives a tolerant tester in the same setting. The work of \cite{SS10} introduces the framework of \emph{local} property reconstruction, which is the same framework our approach uses (i.e. local correction by memoryless LCA). They give a local corrector for functions over the hypergrid $[d]^n$, with large dependence on the dimension $n$ but small dependence on $d$. Lower bounds for monotonicity correction in other error regimes are given in \cite{BGJ+10, AJMR14}. 
The problem of approximating the distance to monotonicity, which is strongly related to tolerant testing, has been studied in \cite{pallavoor2022approximating, ACCL07, Parnas2004TolerantPT}. 

A proper learning algorithm for a function class that generalizes monotone functions is given in \cite{CanonneGG0W16}.
Proper learning of restricted classes of monotone functions has been studied in \cite{Servedio2009OnTL,Ang88,YBC13,Servedio2009OnTL, Blanc2022ProperlyLD}. 
The question of weak learning of monotone functions has also received attention \cite{KearnsV89,bshouty1996fourier,BlumBL98,AmanoM02,ODonnellW09}. The latter line of work investigates proper learning algorithms that have very fast run-time at the cost of having accuracy of only $\frac{1}{2}+\frac{1}{\poly(n)}$.

In addition to the Boolean cube, testing monotonicity has also been studied on hypergrids, see for example
\cite{ChakrabartyS13a},
\cite{BlaisRY14}
\cite{ChakrabartyS13},
\cite{BlackCS18},
\cite{BlackCS20}. Also see
\cite{ChakrabartyS19}
for monotonicity testing of functions with bounded influence.

%\cite{blais2015learning}.

\subsection{Organization of this paper}
In \Cref{sec:LCA} we define the LCA model and state the maximal matching result of \cite{Ghaffari22}.
In \Cref{sec:main} we state and prove the main proper learning and testing results as consequences of our local poset sorting algorithm. 
In \Cref{sec:sorting} we present pseudocode for the local sorting algorithm and analyze its correctness and complexity.






==> Monotone corrector new arxiv version/local_corrector.tex <==

\section{The local corrector.}

The following is true from existing work:
\begin{theorem}
\label{theorem: LCA for maximal independent set}
For any positive constant $C$ the following is true.
Suppose we are given a graph of $N$ vertices with all vertex degrees at most $\Delta$, accessed via an adjacency list oracle (i.e. when queried $(v,j)$ with $v$ a vertex and $j$ an index, the oracle outputs the unique ID of the $j$-th neighbour of $v$, or $\perp$ otherwise). There is an LCA for computing a maximal independent set for this graph that requires $2^{\polylog (\Delta)}\,\polylog (N)$  oracle queries and run-time for each LCA query, with utilization of $2^{\polylog (\Delta)}\,\polylog (N)$ common randomness in total and success\footnote{In the context of LCAs, by the success probability we mean probability of \textbf{global} success of the algorithm. I.e. if one were to make every single query available, then the aggregate result thus obtained would satisfy the required specifications with given probability.} probability at least $1-\frac{1}{N^{C}}$.
\end{theorem}

\begin{corollary}
\label{corollary: can do local maximal matching}
For any positive constant $C$ the following is true.
Suppose we are given a graph of $N$ vertices (not necessarily bipartite) with all vertex degrees at most $\Delta$, accessed via an adjacency list oracle (i.e. when queried $(v,j)$ with $v$ a vertex and $j$ an index, the oracle outputs the unique ID of the $j$-th neighbour of $v$, or $\perp$ otherwise). Then, there is an LCA for computing a maximal matching\footnote{I.e. when the LCA is queried with an edge $(v_1,v_2)$ it has to answer whether it is to be included in the maximal matching. } for this graph that requires $2^{\polylog (\Delta)}\,\polylog (N)$  adjacency list oracle queries and run-time for each LCA query, with utilization of $2^{\polylog (\Delta)}\,\polylog (N)$  common randomness in total and success probability at least $1-\frac{1}{N^{C}}$.
\end{corollary}
\begin{proof}
Let $H$ be the following graph:
\begin{itemize}
    \item There is a vertex in $H$ for every edge in our original graph. In addition to these, there are $N$ extra vertices\footnote{We add these to boost success probability.}
    \item The added extra vertices have no edges adjacent to them.
    \item For two edges $e_1$ and $e_2$ in the original graph, there is an edge in $H$ between the vertices corresponding to $e_1$ and $e_2$ if and only if $e_1$ and $e_2$ share an endpoint in our original graph.
\end{itemize}

We observe that this resulting graph $H$ has at most $2N$ vertices and maximum degree at most $2\Delta$. Furthermore, we can simulate a single adjacency list query for $H$ using $O(\Delta)$ adjacency list queries to our original graph (all neighbours of a vertex $v$ in $H$ can be retrieved by  (i) first checking if it is any of the extra vertices and if so returning $\perp$ (ii) considering the endpoints of the edge corresponding to $v$ in our original graph (iii) using the adjacency list of our original graph to find all the edges adjacent to these neighbours in our original graph). 

We see immediately from definitions that a maximal independent set on $H$ corresponds to a maximal matching on our original graph. Since an adjacency list query on $H$ can be simulated with $O(\Delta)$ overhead via adjacency list queries on our original graph, we therefore get a maximal matching algorithm on our original graph using $\Delta\,2^{\polylog (O(\Delta))}\,\polylog (O(N))=2^{\polylog (\Delta)}\,\polylog (N)$  adjacency list oracle queries and run-time for each LCA query, with utilization of $2^{\polylog (\Delta)}\,\polylog (N)$  common randomness in total and success probability at least $1-\frac{1}{N^{C}}$.


\end{proof}
Now, consider a poset consisting of elements $\{v_i\}$, and we use the symbols $\prec$ and $\succ$ to denote dominance on the poset, as well as symbols $\precimm$ and $\succimm$ to denote immediate predecession and succession\footnote{$v_i\precimm v_j$ if  $v_i\prec v_j$ and there is no element of the poset $u$ satisfying $v_i\prec u \prec v_j$, conversely for $v_i\succimm v_j$}.

We consider the problem of locally correcting a function $f:\:\{v_i\}\rightarrow \{0,1\}$ to make it monotone. Specifically, we would like to provide local access to a monotone function $g$ such that\footnote{For $\{0,1\}$-valued functions $g_1$ and $g_2$, we use the notation $\norm{g_1-g_2}$ to denote the fraction of poset elements on which these two functions disagree.} 
\[
\norm{f-g}\leq O\left(\min_\text{monotone $h$}\norm{f-h}\right).
\]

Suppose the poset has $N$ elements and each element has at most $\Delta$ immediate predecessors and successors. We are given access to the poset via an adjacency-list-like oracle to the immediate predecessors and successors of a given poset element\footnote{It would make sense to also get a comparison oracle, but that seems that does not seem to be needed in the algorithm we are using.}. We are also given an oracle access to the function $f$ we would like to correct. The LCA would provide query access to a corrected function $g$.

Consider the following procedure (henceforth referred to as \textbf{the correcting procedure}) for a given parameter $r$:
\begin{itemize}
    \item Initialize $h_0=f$.
    \item For $i\in \{1,\cdots,r\}$ steps:
    \begin{itemize}
        \item Form a graph $G_i$ whose vertices are the poset elements, and edges are between pairs $v,u$ for which $v\precimm u$ but $h_i(v)=1$ and $h_i(u)=0$.
        \item Obtain a maximal matching $M_i$ over $G_i$.
        \item Form a function $h_{i+1}$ by:
        \begin{itemize}
        \item If an element $v$ of the poset has no edge in the matching $M_i$ adjacent to it, then $h_{i+1}(v)=h_i(v)$. 
            \item For every edge $(u,v)$ in the maximal matching in $G_i$, with $v\precimm u$ set\footnote{I.e. take the direct opposite of what $h_i$ was taking on these elements.} $h_{i+1}(v)=0$ and $h_{i+1}(v)=1$.
        \end{itemize}
    \end{itemize}
\item    Output the function $g=h_r$.
\end{itemize}

\begin{definition}
We say that the poset is $r$-good if irrespective of the initial $\{0,1\}$-valued function $f$ and the choice of matching in each step of the main loop of the algorithm above, the final function $g=h_r$ is monotone. 
\end{definition}

\begin{claim} For any positive constant $C$ the following is true.
It the setting explained above ($N$ total poset elements, at most $\Delta$ immediate predecessors and successors for each element), suppose the poset is $r$-good, and we are given oracle access to a function $f$ on the poset, as well as oracle access. Then there is an LCA that upon query gives oracle access to a monotone function $g$ over the poset for which
\[
\norm{f-g}\leq 2\min_\text{monotone $h$}\norm{f-h}.
\]
Furthermore, each LCA query
requires only $2^{r\,\polylog (\Delta)}\,(\polylog (N))^r$  oracle queries and run-time. In total, $r\,2^{\polylog (\Delta)}\,\polylog (N)$ bits of common randomness is utilized. Success probability is at least $1-\frac{r}{N^{C}}$.
\end{claim}
\begin{proof}
The algorithm simulates correcting procedure, while utilizing the maximal matching algorithm in Corollary \ref{corollary: can do local maximal matching} to compute the matching $M_i$ at each step. The probability that this local algorithm succeeds at all $r$ iterations is at least $1-\frac{r}{N^C}$, which we assume henceforth. As each iteration utilizes $2^{\polylog (\Delta)}\,\polylog (N)$  common randomness, the total amount of common randomness utilized is $r2^{\polylog (\Delta)}\,\polylog (N)$.

We first go about showing that the guarantee $\norm{f-g}\leq 2\min_\text{monotone $h$}\norm{f-h}$ will holds. Since the poset is $r$-good (and since the matching algorithm succeeds in all $r$ iterations), the resulting function $g$ will be monotone. Furthermore, one can get from $f$ to $g$ via flipping a sequence of violated immediate successor-predecessor pairs.\footnote{We say a successor-predecessor pair $(u,v)$ with $u\succimm v$ is violated for a function $h$ if $h(u)<h(v)$. To flip this pair means to change the function $h$ to a new function 
$h'(x)=\begin{cases}h(u)&\text{if $x=v$},\\
h(v)&\text{if $x=u$},\\
h(x)&\text{otherwise}
\end{cases}$.} This is true, because at each iteration of the algorithm a whole set of such successor-predecessor pairs are flipped in this manner (sequence of flipping does not matter as no two of these pairs share an element). 

Now, let $h^*\in \argmin_\text{monotone $h$}\norm{f-h}$ and Let $h_\text{track}$ track the function as it changes from $f$ to $g$ via flipping of violated successor-predecessor pairs. We observe as a successor-predecessor pair $(u,v)$ is flipped, the value of $\norm{h_\text{track}-h^*}$ can only decrease (this follows by recalling that $h^*$ is monotone and then considering all the possibilities for the pair of values $h^*$ takes on $u$ and $v$). Altogether, this means that $\norm{g-h^*}\leq \norm{f-h^*}$ which by triangle inequality implies $\norm{g-f}\leq 2\norm{f-h^*}=2\min_\text{monotone $h$}\norm{f-h}$ as required.

We claim one can compute a value of $h_{i+1}$ with $2^{\polylog (\Delta)}\,\polylog (N)$ queries to values of $h_i$ and run-time expenditure. Indeed:
\begin{itemize}
    \item For an edge $(v_1,v_2)$ (with $v_1\precimm v_2$) determining if it is in $G$ takes only two queries to $h_i$ (i.e. query $h_i(v_1)$ and $h_i(v_2)$ and say "yes" if $h_i(v_1)> h_i(v_2)$) .
    \item  To get all the neighbours of vertex $v$ in $G_i$, one can go through all (at most $2\Delta$) its immediate successors and predecessors (in the poset) and for each of them, determine if the edge connecting it with $v$ is in $G_i$. This takes $O(\Delta)$ queries to $h_i$. (Clearly, this  allows us to get the $j$-th neighbour of $v$ in $G$ as well for a given $j$.)
    \item To determine if an edge $(v_1,v_2)$ is in $M_i$ one needs at most $2^{\polylog (\Delta)}\,\polylog (N)$ adjacency list queries (of $G_i$) and run-time as per Corollary \ref{corollary: can do local maximal matching}. This boils down to $2^{\polylog (\Delta)}\,\polylog (N)$ run-time and queries to $h_i$ (the extra $O(\Delta)$ factor can be absorbed into the constant in the exponent).
    \item To determine the value of $h_{i+1}$ on a given vertex $v$, it is enough to query $h_i(v)$ and determine whether any of the (at most $2\Delta$) adjacent edges in is $M_i$. As per the previous bullet point, this takes $2^{\polylog (\Delta)}\,\polylog (N)$ run-time and queries to $h_i$ (again, the extra $O(\Delta)$ factor can be absorbed into the constant in the exponent).
\end{itemize}

Now, we come back to our original measure of resource consumption: total run-time together with oracle queries to $f$ and the immediate predecessor/successor oracle for the poset.
Clearly, computing a value of $h_0$ on a given element takes $O(1)$ oracle queries and run-time (since $h_0=f$. Therefore, computing a value of $h_i$ on a given element takes $2^{i\,\polylog (\Delta)}\,(\polylog (N))^i$ oracle queries and run-time, giving us the desired $2^{r\,\polylog (\Delta)}\,(\polylog (N))^r$ oracle queries and run-time bound for computing a value of $h_r$.

\end{proof}



==> Monotone corrector new arxiv version/main_result_and_consequences.tex <==
\section{Main result and consequences}
\label{sec:main}

We first present the formal statement for our LCA for the poset sorting problem, from which every other result in this section is derived. The algorithm and analysis are presented in \Cref{sec:sorting}. 
\begin{restatable}{theorem}{main}
\label{thm: the local corrector for general posets}
Let $P$ be a poset of $N$ elements and height $h$, such that each element in $P$ has at most $\Delta$ predecessors or successors.
Suppose we are given query access to the graph of $P$, i.e. for any $x \in P$ we can obtain the immediate predecessors or successors of $x$.
Also, suppose we are given query access to some Boolean function $f$ over $P$.
Then, there is an LCA that solves the poset-sorting problem for $f$ over $P$: in other words, it provides query access to a monotone function $f_{mon}: P \to \zo$ that can be obtained from $f$ by a sequence of swaps of monotonicity-violating label pairs.
The LCA has query complexity and run-time of $\left(\Delta \log\left(\frac{N}{\delta}\right)\right)^{O(\log h)}$, and it uses a random bit-string of length $\poly(\Delta \log \frac{N}{\delta})$.
%Then, there is an LCA giving access to some monotone $f_\text{mon}:P\rightarrow \{0,1\}$, such that the distance between $f$ and $f_\text{mon}$ is at most twice the distance of $f$ to any monotone Boolean function over $P$.. 
%The LCA also has the following extra property. For any monotone $q:P\rightarrow  \{0,1\}$ we have $\norm{f_\text{mon}-q} \leq \norm{f-q}$.
The failure probability of the LCA is at most $\delta$.

\end{restatable}


\begin{restatable}{remark}{refinement remark}
\label{remark: run-time refinement}
In the setting of Theorem \ref{thm: the local corrector for general posets}, 
suppose each element of $P$ has at most $n$ immediate predecessors or successors,
and furthermore, that $P$ is graded 
(all paths between $u$ and $v$ for any $u,v$ have the same length). 
Then query complexity and the run-time of our LCA is also bounded by $n^{O(h)}  (\log(N/\delta))^{\log h}$.
\blue{The number of 
random bits used is at most  $n^{O(h)}\polylog(N/\delta)$.}
%suppose further that for some $\{\Delta_i: i\in \{0,\cdots \lceil \log h\rceil\}\}$ each element of $P$ has at most $\Delta_i$ predecessors or successors within distance $\lceil h/2^{i}\rceil$. Then, the query complexity and the run-time of our LCA is also bounded by $\prod_{i=0}^{\lceil \log h\rceil}O\left(\Delta_i\right)$.
In particular, when $P$ is the truncated hypercube $H_\eps^n$ and $\delta = 2^{-10n}$,
the query and time complexity are $n^{O\left(\sqrt{n \log \frac{1}{\eps}}\right)}$.
\end{restatable}

The proof of \Cref{remark: run-time refinement} is given in \Cref{sec: refined local implementation}.

\begin{proposition}[Local correction]
\label{remark: sorting implies local correction}
In the setting of the previous problem, the distance between $f$ and $f_\text{mon}$ is at most twice the distance of $f$ to monotonicity. Furthermore, the following extra property holds: for any monotone $q:P\rightarrow  \{0,1\}$ we have $\norm{f_\text{mon}-q} \leq \norm{f-q}$. 
\end{proposition}
\begin{proof}
We first show the extra property. Recall that $f_\text{mon}$ can be obtained from $f$ via a sequence of swaps of monotonicity-violating labels. Since $q$ is monotone, as a result of every single of this swaps the distance to $q$ will either decrease or stay the same. Overall across all the swaps, this means that $\norm{f_\text{mon}-q} \leq \norm{f-q}$.

Taking $q$ to be the closest monotone function to $f$ and using the triangle inequality, we see that the distance between $f$ and $f_\text{mon}$ is at most twice the distance of $f$ to monotonicity.
\end{proof}
The two corollaries about tolerant testing of monotone functions follow from our theorem above. We note that the success probability of $2/3$ can be improved via repetition to $1-\delta$ at the cost of $\log \left(\frac{1}{\delta}\right)$ multiplicative factor in run-time and query complexity. We also note that the inverse tolerance ratio, given as $0.49$, can be improved to any absolute constant less than $0.5$.

\begin{corollary}[Tolerant testing for the Boolean cube]
\label{cor:cube tester}
Suppose we are given query access to an unknown Boolean function $f$. Then, there is an algorithm that uses $\blue{n^{O\left(\sqrt{n\log\frac{1}{\epsilon}}\right)}}$ queries and run-time, and distinguishes whether the function $f$ is $0.49\epsilon$-close or $\epsilon$-far from monotone.
The failure probability is at most $2/3$.
\end{corollary}
\begin{proof}
%The proof is essentially the same as the one in the previous corollary, except now we use $H^n_{0.001\epsilon}$ as our poset $P$. Since $\{0,1\}^n$ contains only at most $0.001\epsilon$ fraction of elements outside of $H^n_{0.001\epsilon}$, moving from  
%First of all, without loss of generality we can assume $\delta=2/3$, because the error probability can be reduced via repetition.

We use the truncated hypercube $H^n_{0.005\epsilon}$ as our poset when using
Theorem \ref{thm: the local corrector for general posets} (also using the refined run-time of \Cref{remark: run-time refinement}). This allows us to gain query access to a monotone $f_\text{mon}$ on $H^n_{0.005\epsilon}$. Extend $f_\text{mon}$ to all of $\{0,1\}^n$ by setting it to $1$ above the upper truncation threshold and to $0$ below the lower threshold. Clearly, $f_\text{mon}$ is now also monotone on all of $\{0,1\}^n$.

We sample i.i.d. uniformly random elements of $\{0,1\}^n$, evaluate both $f$ and $f_\text{mon}$ on each these elements and obtain an estimate of $\norm{f-f_\text{mon}}$ up to error $0.005\epsilon$. 
If $f$ is $\epsilon$-far from monotone, then the distance $\norm{f-f_\text{mon}}$ is also at least $\epsilon$, so the estimate will be at least $0.995\epsilon$. If $f$ is $0.49 \epsilon$-close to monotone, then there is some monotone function over $H^n_{0.005\epsilon}$ with which $f$ disagrees on at most $0.49\epsilon \cdot 2^n$ elements of $H^n_{0.005\epsilon}$. The guarantee of Theorem \ref{thm: the local corrector for general posets} (via \Cref{remark: sorting implies local correction}) tells us that then $f$ and $f_\text{mon}$ disagree on at most $0.98\epsilon \cdot 2^n$ elements of $H^n_{0.005\epsilon}$. Since there are only at most $0.005\epsilon \cdot 2^n$ elements in  $\{0,1\}^n$ that are not in $H^n_{0.005\epsilon}$, we see that $\norm{f-f_\text{mon}}$ is at most $0.985\epsilon$. Therefore, the estimate will be at most $0.99\epsilon$. Overall, checking if the estimate is greater than $0.992\epsilon$ allows us to distinguish whether $f$ is $\epsilon$-far from monotone or $0.49\epsilon$-close to monotone.


 For the estimation to succeed, we need to evaluate $f$ and $f_\text{mon}$ on $O\left(\frac{1}{\epsilon^2}\right)$ i.i.d. random elements of $\{0,1\}^n$. For the LCA of $f_\text{mon}$ we can set the overall success probability parameter to be $0.1$. A Chernoff bound and union bound argument then shows that overall success probability is at least $2/3$.
 \blue{For $H^n_{0.005\epsilon}$ our parameters are $h=O\left(\sqrt{n\log\frac{1}{\epsilon}}\right)$, $N=O(2^n)$ and each element of the poset has at most $n$ immediate predecessors or successors. Overall, the run-time given by \Cref{remark: run-time refinement} is 
 $
  n^{O\left(\sqrt{n\log\frac{1}{\epsilon}}\right)}.
 $}
 
\end{proof}

\begin{corollary}[Tolerant testing for general posets]
\label{cor:poset tester}
Suppose we are
in the setting of Theorem \ref{thm: the local corrector for general posets}, and we also have access to an oracle giving us i.i.d. uniform elements in $P$. Then, there is an algorithm that uses\\ $\Delta^{O(\log h \log\log \Delta)}\left(\log\left(N\right)\right)^{O(\log h)}\frac{1}{\epsilon^2}$ queries and run-time, and distinguishes whether the function $f$ is $0.49\epsilon$-close or $\epsilon$-far from monotone.
The failure probability is at most $2/3$.
\end{corollary}
\begin{proof}
The proof is similar to the proof of \Cref{cor:cube tester}, and is given in \Cref{sec: proof of cor:poset tester}. %\Cref{sec: proof of cor:poset tester}.
\end{proof}


\begin{theorem}[Proper learnability of monotone functions]\label{thm: proper learning realizable}
There is an algorithm that, for any monotone function $g:\{0,1\}^n\rightarrow \{0,1\}$, given i.i.d. example-label pairs $(x_i,g(x_i))$, with $x_i$ uniform in $\{0,1\}^n$, returns a circuit computing a \textbf{monotone function} $\hat{g}$, such that $\norm{g-\hat{g}}\leq \epsilon$.
The algorithm uses \blue{$n^{O\left(\frac{\sqrt{n}}{\epsilon}\right)}$} samples and run-time and fails with probability at most $1/2^n$.
%The function class of monotone functions over $\{0,1\}^n$ can be \textbf{properly} $\epsilon$-learned using $2^{\tilde{O}\left(\frac{\sqrt{n}}{\epsilon}\right)}\log\left(\frac{1}{\delta}\right)$ samples and run-time under the uniform distribution over $\{0,1\}^n$, where $\delta$ is the failure probability bound.
\end{theorem}

\begin{proof}
The proper learner does the following:
\begin{enumerate}
    \item Use the improper learner in Theorem \ref{thm: bshouty-tamon realizable} with error parameter $\frac{\epsilon}{10}$ and failure probability bound $1/2^{n+1}$. This gives a circuit computing a function $f$ over $\{0,1\}^n$.
    \item Obtain a circuit computing a function $f_\text{mon}:H^n_{\epsilon/10}\rightarrow\{0,1\}$ as follows. The circuit is computed via running the LCA from Theorem \ref{thm: the local corrector for general posets} with accuracy parameter equal to $\frac{\epsilon}{10}$ and failure probability bound equal to $1/2^{n+1}$, and with the oracle calls to a function replaced with an evaluation of the circuit $f$, restricted to $H^n_{\epsilon/10}$. The random bit-string used by the LCA is hard-coded into the circuit for $h$, so that the resulting circuit is deterministic.
    \item Augment the circuit computing $f_\text{mon}$ in order to extend this function into the whole of $\{0,1\}^n$ as follows. If $|x|>\frac{n}{2}+\sqrt{\frac{n}{2}\log \frac{20}{\epsilon}}$ then $f_\text{mon}(x)=1$, and if $|x|<\frac{n}{2}-\sqrt{\frac{n}{2}\log \frac{20}{\epsilon}}$ then $f_\text{mon}(x)=0$.
    \item Output the circuit computing $f_\text{mon}$.
\end{enumerate}
With probability at least $1/2^{n}$ both of the algorithms we invoke succeed, which we will assume henceforth. 

\blue{
Let us discuss the run-time. Step 1 runs in time $n^{O\left(\frac{\sqrt{n}}{\epsilon}\right)}$ and the circuit for $g$ can therefore only have size at most $n^{O\left(\frac{\sqrt{n}}{\epsilon}\right)}$. For step 2, first observe that we have $\left\lvert H^n_{\epsilon/10} \right\rvert\leq 2^n$, $H^n_{\epsilon/10}$ has height $2\sqrt{\frac{n}{2}\log \frac{20}{\epsilon}}$ and each element in $H^n_{\epsilon/10}$ can have only at most $n$ immediate predecessors and successors. Therefore, the LCA from Theorem \ref{thm: the local corrector for general posets} (refined via \Cref{remark: run-time refinement}) in this setting has run-time, query complexity and bit-string length of $n^{O(\sqrt{n}\log(1/\epsilon))}$. Since the circuit for $f$ itself has size $n^{O\left(\frac{\sqrt{n}}{\epsilon}\right)}$, the overall run-time of the learning algorithm and the size of circuit computing $f_\text{mon}$ is also $2^{O\left(\frac{\sqrt{n}}{\epsilon}\right)}$.}

Finally, we argue correctness. Correctness of the LCA in Theorem \ref{thm: the local corrector for general posets} implies that $f_\text{mon}$ is monotone over $H^n_{\epsilon/10}$ and we see that the extension of this function to $\{0,1\}^n$ in step $3$ keeps it monotone. 

Now, let $g$ be the function we are trying to learn. Since we are in the realizable setting, $g$ is monotone. 
Theorem \ref{thm: bshouty-tamon realizable} tells us that $f$ and $g$ disagree on at most $\frac{\epsilon}{10}2^n$ elements. This, together with Theorem \ref{thm: the local corrector for general posets}, Remark \ref{remark: sorting implies local correction} and the fact that $g$ is monotone, tells us that $f_\text{mon}$ disagrees with $f$ on at most $\frac{\epsilon}{5}2^n$ elements of $H^n_{\epsilon/10}$. The number of $x\in \{0,1\}^n$ not in $H^n_{\epsilon/10}$ is at most $\frac{\epsilon}{10}2^n$, so overall $f_\text{mon}$ disagrees with $f$ on at most $\frac{3\epsilon}{10}2^n$ elements of $\{0,1\}^n$, in other words $\norm{f-f_\text{mon}} \leq \frac{3\epsilon}{10}$. Via triangle inequality, we have $\norm{g-f_\text{mon}} \leq \norm{g-f} +\norm{f-f_\text{mon}} \leq \frac{2\epsilon}{5}\leq \epsilon$, finishing the proof.
\end{proof}
Let us remark on the performance of our algorithm in the agnostic setting.
Observation 3 on page 5 of \cite{kalai_agnostically_2005} implies that the algorithm of \cite{bshouty1996fourier} (i.e. Theorem \ref{thm: bshouty-tamon realizable}), when run in the agnostic setting, will give a predictor with error at most $8\cdot \text{opt}+\epsilon$, where $\text{opt}$ is the error of best monotone predictor. Repeating the argument in the proof of Theorem \ref{thm: proper learning realizable} then tells us that in this setting our proper learning algorithm will also have prediction error $C\cdot \text{opt}+\epsilon$ for some absolute constant $C$. In particular, this means\footnote{Let us elaborate. If we take the error parameter in our algorithm to be $\epsilon/2$, then we see that our algorithm will have prediction error $C \cdot \text{opt}+\epsilon/2$. Then, if noise rate $\text{opt}$ is $\frac{\epsilon}{2C}$ or less, our predictor will be $\epsilon$-competitive with the best monotone function, as required by the agnostic learning model of Kearns, Schapire, and Sellie \cite{kearns1994toward}. } in the agnostic learning model of Kearns, Schapire, and Sellie \cite{kearns1994toward}, our algorithm can handle a noise rate of $\Omega(\epsilon)$. 

We now present how to obtain a better error guarantee in the agnostic setting at a cost of slightly worse dependence of run-time on $\epsilon$:      
\begin{theorem}[Proper learning in agnostic setting]\label{thm: proper learning semi-agnostic}

In the agnostic setting with examples distributed uniformly over $\{0,1\}^n$, 
there is a learning algorithm that outputs a circuit computing a \textbf{monotone function} $\hat{g}$, such that if the best monotone predictor has error $\opt$, then the error of the predictor $\hat{g}$ is at most $3 \cdot \opt +\epsilon$. 
The algorithm uses \blue{$n^{O\left(\frac{\sqrt{n}}{\epsilon} \log\frac{1}{\epsilon}\right)}$} samples and run-time. The failure probability of the algorithm is at most $1/2^n$.
\end{theorem}
\begin{proof}
The proof, presented in  \Cref{sec: proof of thm: proper learning semi-agnostic},
follows a pattern similar to the proof of Theorem \ref{thm: proper learning realizable}. 
\end{proof}


==> Monotone corrector new arxiv version/path_shortening_general.tex <==

Our algorithm works by finding a maximal matching over the $k$-violation graph $B_k$, and swapping the matched labels. We first claim that performing this swap reduces the \red{distance (length of the longest path)} between violated labels by at least $k$.
%We have $\epsilon\in(0,1)$ and we assume it is sufficiently small. We let $H_n$ be the truncated hypercube 
%$$
%H_n:=\fig{x \in \{0,1\}^n:~\abs{\sum_ix_i-\frac{n}{2}}\leq t},
%$$
%where $t:=\sqrt{\frac{n}{2}\log \frac{20}{\epsilon}}$. Via Hoeffding's bound, we have that the fraction of elements in $\{0,1\}^n$ that is not also in $H_n$ is at most $2\exp\left(-\frac{2t^2}{n}\right)=\frac{\epsilon}{10}$.

%\blue{Arsen: I think we should
%do a better job reminding reader that dist is maximum distance.}

\begin{lemma}[Distance shortening lemma]\label{lemma: path shortening lemma}
Let $P$ be any poset. 
Let $f$ be a $\{0,1\}$-valued function over $P$ and $k$ be a positive integer. Let $B_{k}$ be as defined in \Cref{def:viol-graph}. Suppose one picks some maximal matching $M$ over $B_{k}$ and obtains a new function $f'$ as follows
$$
f'(x)=
\begin{cases}
f(x) &\text{if $x$ was not matched},\\
f(y) &\text{if $x$ was matched to some $y$}.
\end{cases}
$$
Then, we have
\begin{align*}
&\max_{(\bv, \bw) \in \viol_P(f')}\dist(v , w) \leq \\
&\max\left(k-1, \left(\max_{(\bv, \bw) \in \viol_P(f)}\dist(v , w)\right) - k \right).
\end{align*}
\end{lemma}
\begin{proof}
Let $\lambda: P \rightarrow P$ map $x$ to (i) $y$ if $x$ was mapped to some $y$ by $M$ (ii) $x$ itself otherwise. Note that $f'(x)=f(\lambda(x))$ and also $\lambda$ is one-to-one. 

Let $x,y$ in $P$ be such that $x\succ y$, $f(x)=0$ and $f(y)=1$. If $\dist(x,y) \geq k$, it cannot be the case that both $\lambda(x)=x$ and $\lambda(y)=y$, because then $M$ would not be a maximal matching since we could also match $x$ to $y$. Besides, note that if $\lambda(x) \neq x$ then $\lambda(x) \prec x$ and  $\dist(x,\lambda(x))\ge k$. Analogously, if $\lambda(y) \neq y$ then $\lambda(y) \succ y$ and  $\dist(y,\lambda(y)) \ge k$. Additionally, for any $a,b,c\in P$ if $a \succ b \succ c$ then $\dist(a,c)\ge \dist(a,b)+\dist(b,c)$, as there exists a path from $a$ to $c$ that is the union of the longest paths from $a$ to $b$ and $b$ to $c$.
Taking these observations together, we see that only following eight cases are possible:
\begin{enumerate}
    \item $\dist(x,y) \leq k-1$.
    \begin{enumerate}
        \item $\lambda(x) \succ \lambda(y)$ and \\ 
        $\dist(\lambda(x),\lambda(y)) \leq \dist(x,y) \leq k-1$.
        \item It is not the case that $\lambda(x) \succ \lambda(y)$.
    \end{enumerate}
    \item $\dist(x,y) \geq k$.
    \begin{enumerate}
    \item $\lambda(x)=x$ and $\dist(y,\lambda(y)\ge k$
    \begin{enumerate}
        \item $\lambda(x) \succ \lambda(y)$ and \\
        $\dist(\lambda(x),\lambda(y))\le \dist(x,y)-k$.
        \item It is not the case that $\lambda(x) \succ \lambda(y)$.
    \end{enumerate}
    \item $\lambda(y)=y$ and $\dist(x,\lambda(x))\ge k$
    \begin{enumerate}
        \item $\lambda(x) \succ \lambda(y)$ and \\
        $\dist(\lambda(x),\lambda(y))\le \dist(x,y)-k$.
        \item It is not the case that $\lambda(x) \succ \lambda(y)$.
    \end{enumerate}
    \item $\dist(x,\lambda(x))\ge k$ and $\dist(y,\lambda(y))\ge k$
    \begin{enumerate}
        \item $\lambda(x) \succ \lambda(y)$ and \\
        $\dist(\lambda(x),\lambda(y))\le \dist(x,y)-2k$.
        \item It is not the case that $\lambda(x) \succ \lambda(y)$.
    \end{enumerate}
    \end{enumerate}
\end{enumerate}
In the whole, if $\lambda(x) \succ \lambda(y)$ then $\dist(\lambda(x),\lambda(y))\leq \max(k-1,\dist(x,y)-k)$.

Now let's consider what happens after the swap. Let $v_0,w_0$ in $P$ maximize $\dist(v_0,w_0)$ subject to $v_0\succ w_0$, $f'(v_0)=0$ and $f'(w_0)=1$. Let $x=\lambda^{-1}(v_0)$ and $y=\lambda^{-1}(w_0)$.
Since $f'(v_0)=0$, we have $x \succeq v_0$ and since $f'(w_0)=1$, we have $y \preceq w_0$. Therefore, $x \succ y$. Also, $f(x)=f'(v_0)=0$, $f(y)=f'(w_0)=1$ and $\lambda(x)\succ\lambda(y)$. The conclusion of the previous paragraph tells us that $\dist(v_0,w_0)= \dist(\lambda(x),\lambda(y)) \leq \max(k-1,\dist(x,y)-k)$. Overall,
\begin{align*}
    &\max_{(v , w)\in\viol_P(f')}\dist(v , w) =  \dist(v_0,w_0) \\
    &\leq \max(k-1,\dist(x,y)-k) \\
    &\leq\max\left(k-1, \left(\max_{(v , w)\in\viol_P(f)}\dist(v , w)\right) - k \right),
\end{align*}
%\begin{multline*}
%    \max_{\viol_P(f)}\dist(v , w) =  \dist(v_0,w_0) \leq \max(k-1,\dist(x,y)-k) \leq\\
%    \leq\max\left(k-1, \left(\max_{\viol_P(f)}\dist(v , w)\right) - k \right),
%\end{multline*}
which finishes the proof.
\end{proof}


==> Monotone corrector new arxiv version/path_shortening_lemma.tex <==

\section{Path shortening lemma}
%We have $\epsilon\in(0,1)$ and we assume it is sufficiently small. We let $H_n$ be the truncated hypercube 
%$$
%H_n:=\fig{\vect{x} \in \{0,1\}^n:~\abs{\sum_ix_i-\frac{n}{2}}\leq t},
%$$
%where $t:=\sqrt{\frac{n}{2}\log \frac{20}{\epsilon}}$. Via Hoeffding's bound, we have that the fraction of elements in $\{0,1\}^n$ that is not also in $H_n$ is at most $2\exp\left(-\frac{2t^2}{n}\right)=\frac{\epsilon}{10}$.

\begin{definition}[High-distance violation graph]
\label{def:viol-graph}
For a graded directed graph $G$ of height $h$, a function $f$ over $V(G)$, and some $d \in [h]$, we define the high-distance violation graph $G_d$ as follows:

\begin{itemize}
	\item $V(G_d) = V(G)$, and 
	\item For $\vect{u}, \vect{v} \in V(G)$, $(\vect{u}, \vect{v}) \in E(G_d)$ iff $\vect{u} \prec_G \vect{v}$, $\dist_G(\vect{u}, \vect{v}) \ge d$, and $f(\vect{u}) > f(\vect{v})$.
\end{itemize}
\end{definition}


\begin{lemma}[Distance shortening lemma]\label{lemma: path shortening lemma}
Let $P$ be a graded poset. 
Let $f$ be a $\{0,1\}$-valued function over $P$ and $k$ be a positive integer. Let $B_{k}$ be a graph whose vertex set is $P$ and two vertices $\vect{v}$ and $\vect{w}$ are connected when both of the following hold (i) $\vect{v}\prec \vect{w}$ and $f(\vect{v})>f(\vect{w})$ or $\vect{v}\succ \vect{w}$ and $f(\vect{v})<f(\vect{w})$ (ii) $\dist(\vect{v}, \vect{w}) \geq k$. Suppose one picks some maximal matching $M$ over $B_{k}$ and obtains a new function $f'$ as follows
$$
f'(x)=
\begin{cases}
f(x) &\text{if $x$ was not matched},\\
f(y) &\text{if $x$ was matched to some $y$}.
\end{cases}
$$
Then, we have
$$
\max_{\vect{v}, \vect{w} \in P: ~ \vect{v}\succ \vect{w},~ f'(\vect{v})=0 \text{ and } f'(\vect{w})=1  }\dist(\vect{v} , \vect{w}) \leq \max\left(k-1, \left(\max_{\vect{v}, \vect{w} \in P: ~ \vect{v}\succ \vect{w},~ f(\vect{v})=0 \text{ and } f(\vect{w})=1  }\dist(\vect{v} , \vect{w})\right) - k \right).
$$
\end{lemma}
\begin{proof}
Let $\lambda: P \rightarrow P$ map $\vect{x}$ to (i) $\vect{y}$ if $\vect{x}$ was mapped to some $\vect{y}$ by $M$ (ii) $\vect{x}$ itself otherwise. Note that $f'(\vect{x})=f(\lambda(\vect{x}))$ and also $\lambda$ is one-to-one. 

Let $x,y$ in $P$ be such that $\vect{x}\succ \vect{y}$, $f(\vect{x})=0$ and $f(\vect{y})=1$. If $\dist(\vect{x},\vect{y}) \geq k$, it cannot be the case that both $\lambda(\vect{x})=\vect{x}$ and $\lambda(\vect{y})=\vect{y}$, because then $M$ would not be a maximal matching since we could also match $\vect{x}$ to $\vect{y}$. Besides, note that if $\lambda(\vect{x}) \neq \vect{x}$ then $\lambda(\vect{x}) \prec \vect{x}$ and  $\dist(\vect{x},\lambda(\vect{x}))\ge k$. Analogously, if $\lambda(\vect{y}) \neq \vect{y}$ then $\lambda(\vect{y}) \succ \vect{y}$ and  $\dist(\vect{y},\lambda(\vect{y})) \ge k$. Additionally, for any $\vect{a},\vect{b},\vect{c}\in P$ if $\vect{a} \succ \vect{b} \succ \vect{c}$ then $\dist(\vect{a},\vect{c}) = \dist(\vect{a},\vect{b})+\dist(\vect{b},\vect{c})$.
Taking these observations together, we see that only following cases are possible
\begin{enumerate}
    \item $\dist(\vect{x},\vect{y}) \leq k-1$.
    \begin{enumerate}
        \item $\lambda(x) \succ \lambda(y)$ and $\dist(\lambda(\vect{x}),\lambda(\vect{y})) \leq \dist(\vect{x},\vect{y}) \leq k-1$.
        \item It is not the case that $\lambda(x) \succ \lambda(y)$.
    \end{enumerate}
    \item $\dist(\vect{x},\vect{y}) \geq k$.
    \begin{enumerate}
    \item $\lambda(\vect{x})=\vect{x}$ and $\dist(\vect{y},\lambda(\vect{y})\ge k$
    \begin{enumerate}
        \item $\lambda(x) \succ \lambda(y)$ and $\dist(\lambda(\vect{x}),\lambda(\vect{y}))\le \dist(\vect{x},\vect{y})-k$.
        \item It is not the case that $\lambda(x) \succ \lambda(y)$.
    \end{enumerate}
    \item $\lambda(\vect{y})=\vect{y}$ and $\dist(\vect{x},\lambda(\vect{x}))\ge k$
    \begin{enumerate}
        \item $\lambda(x) \succ \lambda(y)$ and $\dist(\lambda(\vect{x}),\lambda(\vect{y}))\le \dist(\vect{x},\vect{y})-k$.
        \item It is not the case that $\lambda(x) \succ \lambda(y)$.
    \end{enumerate}
    \item $\dist(\vect{x},\lambda(\vect{x}))\ge k$ and $\dist(\vect{y},\lambda(\vect{y}))\ge k$
    \begin{enumerate}
        \item $\lambda(x) \succ \lambda(y)$ and $\dist(\lambda(\vect{x}),\lambda(\vect{y}))\le \dist(\vect{x},\vect{y})-2k$.
        \item It is not the case that $\lambda(x) \succ \lambda(y)$.
    \end{enumerate}
    \end{enumerate}
\end{enumerate}
In the whole, if $\lambda(x) \succ \lambda(y)$ then $\dist(\lambda(\vect{x}),\lambda(\vect{y}))\leq \max(k-1,\dist(\vect{x},\vect{y})-k)$.

Now let's consider what happens after the swap. Let $\vect{v}_0,\vect{w}_0$ in $P$ maximize $\dist(\vect{v}_0,\vect{w}_0)$ subject to $\vect{v}_0\succ \vect{w}_0$, $f'(\vect{v}_0)=0$ and $f'(\vect{w}_0)=1$. Let $\vect{x}=\lambda^{-1}(\vect{v}_0)$ and $\vect{y}=\lambda^{-1}(\vect{w}_0)$.
Since $f'(\vect{v}_0)=0$, we have $\vect{x} \succeq \vect{v}_0$ and since $f'(\vect{w}_0)=1$, we have $\vect{y} \preceq \vect{w}_0$. Therefore, $\vect{x} \succ \vect{y}$. Also, $f(\vect{x})=f'(\vect{v}_0)=0$, $f(\vect{y})=f'(\vect{w}_0)=1$ and $\lambda(\vect{x})\succ\lambda(\vect{y})$. The conclusion of the previous paragraph tells us that $\dist(\vect{v}_0,\vect{w}_0)= \dist(\lambda(\vect{x}),\lambda(\vect{y})) \leq \max(k-1,\dist(\vect{x},\vect{y})-k)$. Overall,
\begin{multline*}
    \max_{\vect{v}, \vect{w} \in P: ~ \vect{v}\succ \vect{w},~ f'(\vect{v})=0 \text{ and } f'(\vect{w})=1  }\dist(\vect{v} , \vect{w}) =  \dist(\vect{v}_0,\vect{w}_0) \leq \max(k-1,\dist(\vect{x},\vect{y})-k) \leq\\
    \leq\max\left(k-1, \left(\max_{\vect{v}, \vect{w} \in P: ~ \vect{v}\succ \vect{w},~ f(\vect{v})=0 \text{ and } f(\vect{w})=1  }\dist(\vect{v} , \vect{w})\right) - k \right),
\end{multline*}
which finishes the proof.
\end{proof}


==> Monotone corrector new arxiv version/preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelim}

\subsection{Notation (posets and distances)}

Let $x$ and $y$ be elements of a poset $P$.\footnote{In this work all posets are assumed to be finite.} We use $\preceq$ to denote the ordering relation on $P$. We say $x\prec y$ (``$x$ is a predecessor of $y$'') if $x\preceq y$ and $x\neq y$. Also, we say $x\succeq y$ if $y\preceq x$, and $x\succ y$ (``$x$ is a successor of $y$'') if $y\prec x$. We say $x$ and $y$ are \emph{incomparable} if neither $x\prec y$ nor $x\succ y$ holds.
We say that $x$ is an \emph{immediate predecessor} of $y$ if $x\prec y$ and there is no $z$ in $P$ for which $x\prec z \prec y$. The notion of an \emph{immediate successor} is defined analogously.
%\begin{definition}
%A \textbf{poset} (short for \textbf{partially ordered set}) $P$ is a finite\footnote{One can also consider infinite posets, but in this work all our posets will be finite.} set equipped with with a relation $ \preceq $, which has the following properties: (i) \textbf{reflexivity} $x\preceq x$ for any $x$ in $P$ (ii) \textbf{transitivity}: if $x \preceq y$ and $y \preceq z$, then $x\preceq z$ (iii) \textbf{anti-symmetry} if $x \preceq y$ and $y \preceq x$, then $x=y$.
%\end{definition}

The \emph{graph} of a poset $P$ (a.k.a. \emph{Hasse diagram} of $P$) is a directed graph, in which elements of $P$ are the vertices, and there is an edge from $x$ to $y$ whenever $x$ is an immediate predecessor of $y$. 
Clearly, the graph of any poset is a DAG. Additionally, it is immediate that the poset itself is unambiguously determined by its graph, and we will refer to the poset and its graph interchangeably. 
\begin{definition}[Graph distance and height]
We will write $\dist(x,y)$ to denote the length of the \textbf{longest} directed path\footnote{If $x$ and $y$ are incomparable, then $\dist(x,y)$ is undefined.} between $x$ and $y$ in the Hasse diagram of $P$. The \textbf{height} of a poset $P$ is the length of the longest directed path between any two elements in $P$. 
\end{definition}
%\begin{definition}
%A function $f:P\rightarrow \{0, 1\}$ is \emph{monotone} if whenever $x\preceq y$ we have $f(x)\le f(y)$.
%\end{definition}
\begin{definition}[Function distance]
For a pair of functions $f_1, f_2: P\rightarrow \{0, 1\}$, the \textbf{distance} $\norm{f_1-f_2}$ is the fraction of elements $x$ in $P$ on which $f_1(x)\neq f_2(x)$.
\end{definition}
\begin{definition}[Distance to monotonicity]
For a function $f:P\rightarrow \{0, 1\}$, the \textbf{distance to monotonicity} is defined as $\min_{\text{monotone Boolean }f'}\left(\norm{f-f'}\right)$.
\end{definition}
\subsection{Agnostic learning setting}

Now, we formally describe the setting of agnostic learning under the uniform distribution. The learning algorithm is given i.i.d. example-label pairs from some distribution over $\{0,1\}^n \times \{0,1\}$, where the marginal distribution over examples is uniform. The \emph{generalization error} (which we also refer to simply as \emph{error}) of a predictor is the probability it misclassifies a fresh example-label pair. The goal of agnostic learning is to produce a predictor $\hat{g}$ with good generalization error. Guarantees are produced in terms of the lowest generalization error among all hypotheses in the function class (in our case monotone functions), which we denote as $\opt$.


%We are working over some set $U$. Let $\mathcal{F}$ be a \emph{function class}, i.e. a set of functions $U\rightarrow \{0, 1\}$. $D$ will always be a distribution over $U$.

\subsection{The LCA model}
\label{sec:LCA}
%\red{
%\begin{definition}[Local computation algorithm]
%A \emph{Local Computation Algorithm} (LCA)\footnote{This setting is sometimes also 
%called \emph{parallelizable LCA}.} 
%$\mathcal{L}$ takes an element from 
%some set $A$ and outputs an element in some set $B$.  
%Often times, the LCA is also given access to an oracle $\mathcal{O}$ (or multiple oracles). 
%The algorithm also has query access to a uniformly random bit-string. 
%We say that the LCA \emph{succeeds} if the map $A \rightarrow B$ given by the algorithm (which in general depends on the random bit-string) has the desired property, 
%which can depend on the object given by the oracle.
%\end{definition}}

The Local Computation Algorithm (LCA) model captures the 
ability to provide query access to parts of an output in sublinear time.
In this work, we use the LCA model for the 
problems of maximal matching and 
poset sorting.   
An LCA is given access to a random bit-string
and to the input:  
for example, in the case of maximal matching,
this input is the adjacency list of the graph.
%For maximal matching on input graph $G$, 
Upon receiving an edge query $e$ in $G$,
the LCA should respond ``yes'' or ``no.''
%a query to the LCA is any edge $e$ in $G$,
%and the LCA, which is provided with
%access to the adjacency list of $G$, responds with whether $e$ is
%in $M$ in sublinear time. 
%The output of the
%LCA may depend on a random bit-string.  
Responses to different
edges must be consistent with a single legal
maximal matching.  
Similarly, for poset sorting on poset $P$, 
a query to the LCA is any element $x \in P$, 
and the LCA, which is provided with access to
function $f:P \rightarrow \{0,1\}$, must respond with  $f_{\text{mon}}(x)$ so that
the function $f_{\text{mon}}$ is monotone.
%function that is (hopefully) close 
%to $f$.
Responses to different inputs must be consistent with 
a single legal sorting of $f$.
In both cases,  the LCA's answers
may depend on a random
bit-string\footnote{In all cases we consider, the random bit-string is short enough for the LCA to read as a whole (in contrast, in some work exponentially long bit-strings are considered). 
} that persists between queries, but otherwise, responses must be\footnote{Sometimes LCAs are considered that are not memoryless, but in this work whenever we refer to an LCA, we imply it is memoryless.}
{\em memoryless} -- i.e., they cannot depend on previous queries to or responses
from the LCA. 


%\red{Let us consider a concrete example: maximal matching on a graph. Here, the oracle $\mathcal{O}$ gives access to some graph (for a queried node, one gets its neighbors). $A$ is the set of node pairs in the graph, $B$ is $\{0,1\}$ and the mapping $A\rightarrow B$ indicates whether a given edge is included in the matching. The LCA succeeds if the set to which it gives implicit access is (a) a subset of edges in the graph, (b) a matching, and (c) maximal (i.e. there is no edge available to be added to it).} 
%
In terms of performance, we want the following quantities to be as small as possible (i) the \emph{query complexity}, i.e. the number of probes to the input the LCA makes to respond to a single query, (ii) the \emph{run-time} the LCA needs to respond to a query, (iii) the length of the random bit-string used by the LCA, (iv) the probability over the random bit-string that the LCA fails to satisfy the problem specifications. 

We will use a recent powerful result\footnote{We need to comment on some superficial differences between Theorem \ref{thm: Ghaffari Uitto LCA theorem} and the main theorem of \blue{\cite{Ghaffari22}}, which does not mention run-time and bit-string length explicitly and also has \blue{$\delta=\poly\left(\frac{1}{N}\right)$}. The following observations are not novel in any way, and some of them are alluded to in \blue{\cite{GhaffariU19, Ghaffari22}}, but we explain them here for completeness.
The bound on run-time follows by direct inspection of their algorithm. 
The length of the bit-string can be reduced to \blue{$
\poly(\Delta, \log(N/\delta))$} via the standard method \cite{AlonRVX12,levi_local_2015} of replacing i.i.d. random bits with $k$-wise independent random bits for $k$ large enough ($k=\blue{
\poly(\Delta, \log(N/\delta))}$ suffices, as number of those i.i.d. random bits accessed per query is \blue{$
\poly(\Delta, \log(N/\delta))$}). Although, the failure probability bound $\delta$ in the original theorem of \cite{Ghaffari22} is set to be \blue{$\poly\left(\frac{1}{N}\right)$}, it can be boosted to arbitrary $\delta$ by adding extra disconnected vertices to our graph until \blue{this value reaches} $\delta$ for the new number of vertices $N'$. Query access to this new graph can be simulated via query access to the original graph with inconsequential overhead. Overall, this costs one an extra $\polylog(1/\delta)$ factor in
query complexity and run-time.
}
of \blue{Ghaffari \cite{Ghaffari22}}, which gives an efficient algorithm for answering membership queries to a maximal independent set. (We emphasize that \emph{maximal} independent set is defined to be an independent set that cannot be made into a larger independent set by adding an extra vertex, and \emph{maximal matching} is defined analogously.) \blue{We note that
in an earlier version of this paper (which was written before \cite{Ghaffari22} was available) we used the theorem of Ghaffari and Uitto  \cite{GhaffariU19} for this purpose.   }
\begin{theorem}[\blue{\cite{Ghaffari22}}]\label{thm: Ghaffari Uitto LCA theorem}
There is an LCA that takes all-neighbor\footnote{I.e. when queried a vertex $v$, the oracle returns all the neighbors of $v$.} access to a graph $G$ with $N$ vertices and largest degree at most $\Delta$, and gives membership access to a \emph{maximal independent set} on the graph. The query complexity and the run-time of the LCA are \blue{$
\poly(\Delta, \log(N/\delta))$}, the length of the random bit-string is also \blue{$
\poly(\Delta, \log(N/\delta))$} and the failure probability is at most $\delta$.
\end{theorem}

 
 
\begin{corollary}
\label{cor:matchings}
There is an LCA that takes all-neighbor access to a graph $G$, with $N$ vertices and largest degree at most $\Delta$, and gives membership access to a \emph{maximal matching} on the graph. The query complexity and the run-time of the LCA is \blue{$
\poly(\Delta, \log(N/\delta))$}, the length of the random bit-string is also \blue{$
\poly(\Delta, \log(N/\delta))$} and the failure probability is at most $\delta$.
\end{corollary}
\begin{proof}
This reduction is standard; see \Cref{sec: proof of cor:matchings} for details.%\Cref{sec: proof of cor:matchings}.
\end{proof}
%\begin{definition}[Local computation algorithms]  
%\end{definition}

%\begin{definition}
%An algorithm is an \emph{$\epsilon$-learner for the function class $\mathcal{G}$} with failure probability bound $\delta$ under distribution $D$ if the following holds. For any $g \in \mathcal{G}$, given access to samples $(x_i,g(x_i))$ with $x_i$ i.i.d. from $D$, the algorithm with probability at least $1-\delta$ outputs a predictor circuit $\hat{g}$ for which $\Pr_{x \in_R D}\left[g(x)\neq \hat{g}(x)\right]\leq \epsilon$.
%\end{definition}
%
%\begin{definition}
%For $\alpha\geq 1$,
%an algorithm is an \emph{$\alpha$-semiagnostic $\epsilon$-learner for the function class $\mathcal{G}$} with failure probability bound $\delta$ under distribution $D$ if the following holds. Suppose the algorithm is given access to i.i.d. samples $(x_i,y_i)$ from a distribution $D_\text{pairs}$, such that $x_i$ themselves are distributed according to $D$.
%Then, the algorithm with probability at least $1-\delta$ outputs a predictor circuit $\hat{g}$ for which 
%$$\Pr_{(x,y) \in_R D_\text{pairs}}\left[\hat{g}(x)\neq y\right] \leq 
%\alpha \min_{g\in \mathcal{G}} \Pr_{(x,y) \in_R D_\text{pairs}}\left[g(x)\neq y\right] + \epsilon.$$
%\end{definition}
%\noindent Sometimes the name \emph{weakly agnostic} is used in place of semiagnostic. If $\alpha=1$, such algorithm is said to be (fully) \emph{agnostic}. 
%
%\begin{definition}
%In the definitions above, if one also requires that $\hat{f}$ be in $\mathcal{F}$, then the learning algorithm is said to be \emph{proper}.
%\end{definition}
\subsection{Boolean hypercube.}
\begin{definition}
The \emph{$n$-dimensional Boolean hypercube} is the set $\{0,1\}^n$.
For $x,y\in \{0,1\}^n$, we say $x\preceq y$ if for all $i\in\{1,\cdots,n\}$ one has $x_i\leq y_i$. It is immediate that $\{0,1\}^n$ is a poset with $2^n$ elements. 

We also define the truncated hypercube 
$$
H^n_\epsilon:=\fig{x \in \{0,1\}^n:~\abs{\sum_ix_i-\frac{n}{2}}\leq \sqrt{\frac{n}{2}\log \frac{2}{\epsilon}}},
$$
Via Hoeffding's bound, we have that the fraction of elements in $\{0,1\}^n$ that are not also in $H_n^\epsilon$ is at most $2\exp\left(-\frac{2t^2}{n}\right)=\epsilon$.
\end{definition}

\textbf{Known results about learning monotone functions over Boolean hypercube.}
\begin{theorem}[Learnability of monotone functions \cite{bshouty1996fourier}]\label{thm: bshouty-tamon realizable}
There is an algorithm that, for any monotone function $g:\{0,1\}^n\rightarrow \{0,1\}$, given i.i.d. example-label pairs $(x_i,g(x_i))$, with $x_i$ uniform in $\{0,1\}^n$, returns a circuit computing a predictor $\hat{g}$, such that $\norm{g-\hat{g}}\leq \epsilon$.
The algorithm uses $\blue{n^{O\left(\frac{\sqrt{n}}{\epsilon}\right)}}\log\left(\frac{1}{\delta}\right)$ samples and run-time, where $\delta$ is the failure probability bound.
\end{theorem}


The standard theorem below follows via low-degree concentration result of \cite{bshouty1996fourier}, Remark 4 on page 6 of \cite{kalai_agnostically_2005}, the refinement\footnote{We note that in an earlier version of this work we were not aware of the refinement of \cite{feldman_tight_2020}, so the $\epsilon$-dependence in the \Cref{thm: bshouty-tamon agnostic}, as well as in \Cref{thm: proper learning semi-agnostic}, was slightly worse.} of \cite{feldman_tight_2020} and standard failure probability reduction via repetition. Please refer to \Cref{sec: best improper  agnostic learning algorithm from the literature.} for more detail.
\begin{theorem}[Agnostic learnability of monotone functions]\label{thm: bshouty-tamon agnostic}
In the agnostic setting with examples distributed uniformly on $\{0,1\}^n$, there is an algorithm that returns a circuit with generalization error at most $\textnormal{opt}+\epsilon$, where $\textnormal{opt}$ is the error of the best monotone function. The algorithm uses $\blue{n^{O\left(\frac{\sqrt{n}}{\epsilon}\log \frac{1}{\epsilon}\right)}}\log\left(\frac{1}{\delta}\right)$ samples and run-time, where $\delta$ is the failure probability bound.

\end{theorem}


==> intro.tex <==
\input{abstract}
\section{Introduction}
%\subsection{Main result: proper learning of monotone functions.}

\paragraph{Proper learning of monotone functions.} Consider the \emph{proper learning} problem for monotone functions:
\begin{center}
\textit{
Given i.i.d uniform labeled examples from an unknown monotone $g:\{0,1\}^n\rightarrow \{0,1\}$, output a predictor computing monotone $\hat{g}:\{0,1\}^n\rightarrow \{0,1\}$ that predicts $g$ correctly on at least $1-\epsilon$ fraction of the domain. 
}
\end{center}
For over 25 years there has been a large statistical-to-computational gap in our understanding of this problem. 
A $2^{\tilde{O}(\sqrt{n}/\eps)}$-time \emph{improper} learning algorithm --- that is, an algorithm that outputs a predictor $f$ that is accurate but not guaranteed to be monotone --- is given in \cite{bshouty1996fourier}.
%\gray{Specifically, the work of \cite{bshouty1996fourier} gives a $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$-time algorithm for obtaining a predictor $f$ that itself is not guaranteed to be monotone (such learner is called \textbf{improper}).}
One could use the output of this algorithm to 
obtain a monotone $\hat{g}$ by computing $f$ on every element of $\{0,1\}^n$ and solving a linear program to obtain the closest monotone function to $f$. Although this gives a $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$-sample algorithm, the run-time is $2^{\Omega(n)}$. No proper learning algorithm with faster run-time was known.

Through a new connection with local computation algorithms, we close this gap by giving a $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$-time algorithm for this problem. Note that the running time essentially matches that of the aforementioned improper learning algorithm of \cite{bshouty1996fourier}. Moreover, our algorithm is essentially optimal, due to the $2^{\Tilde{\Omega}(\sqrt{n})}$ query lower bound of \cite{blais2015learning}. 
Furthermore, our algorithm is robust to adversarial noise in the labels. Specifically, in the agnostic learning model of Kearns, Schapire, and Sellie \cite{kearns1994toward}, our algorithm can handle a noise rate of $\Omega(\epsilon)$.     

\paragraph{Monotonicity testing.}
The question of testing monotonicity of an unknown Boolean function over $\{0,1\}^n$ (given query access) has received a large amount of attention  
\cite{goldreich_testing_1998,chakrabarty_on_2013,chen_new_2014,chen_boolean_2015,khot_monotonicity_2015,belovs_polynomial_2016,chen_beyond_2017}. However, the algorithms in this line of work possess the drawback of having a large \emph{tolerance ratio}\footnote{A tester for monotonicity distinguishes a monotone function from a function that is $\epsilon$-far from monotone.
In this work, we use tolerance ratio $\alpha$ to  mean that the tester will accept a function $\epsilon/\alpha$-close to monotone.}, i.e. they will reject some functions that are extremely close to monotone. The more recent work of \cite{pallavoor2022approximating} gives a tester with tolerance ratio of $\tilde{O}(\sqrt{n})$, and this is the best tolerance ratio known\footnote{Note that Theorem 1.8 of \cite{CanonneGG0W16} gives a $2^{o(n)}$-query algorithm (no run-time bound is claimed). The run-time is still $2^{\Omega(n)}$ due to step 8 of their Algorithm 2 on page 31.} for a $2^{o(n)}$-run-time algorithm.  

As a simple corollary of our proper learning algorithm,
one can already achieve \emph{constant tolerance ratio for monotonicity testing with  $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$ run-time} via a well-known connection between learning and testing \cite{goldreich1998property}. (We emphasize that, to draw this corollary, it is critical that the learning algorithm is proper and robust to noise in labels.) Further, building more directly on our technical ideas, we present a constant-tolerance monotonicity tester with \emph{exponentially better dependence on $\epsilon$ of $2^{\Tilde{O}\left(\sqrt{n \log \frac{1}{\epsilon}}  \right)}$}. This approach also yields a tolerant tester for functions over general posets, which we describe in detail in \textbf{todo: link section}. 

%The work of \cite{} builds upon this line of work to give an algorithm of tolerance ratio of $\tilde{O}(\sqrt{n})$
%are not guaranteed to be \textbf{tolerant}\footnote{A regular tester for monotonicity distinguishes between monotone functions and functions $\epsilon$-far from monotone. A \textbf{tolerant} tester for monotonicity for some absolute constant $C$ distinguishes functions that are $\epsilon/C$-close to monotone from functions $\epsilon$-far from monotone.}. In fact, these algorithms could reject functions as close as $\frac{\epsilon}{\poly(n)}$ to monotone.
%Through a well-known connection between learning and testing \cite{goldreich1998property}, as a corollary of our result we obtain a $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$-time \textbf{tolerant tester for monotonicity} of an unknown function $g:\{0,1\}^n\rightarrow \{0,1\}$. In other words, for some absolute constant $C$, in time $2^{\Tilde{O}\left(\sqrt{n}/\epsilon \right)}$ we can test if $g$ is $\frac{\epsilon}{C}$-close to monotone or $\epsilon$-far from monotone. Here also,
%no algorithm with non-trivial run-time was known previously. We emphasize that to draw this corollary it is critical that the learning algorithm is proper (robustness to noise in labels is also important).  


%Over the years, the study of monotone Boolean functions over the Boolean cube has been an important direction in our field. 
%\textbf{todo: cite O'Donnell book?} 



\subsection{Monotonicity correction via sorting on partially ordered sets.}
%\textbf{todo: list of cites on local correction} Our core idea is a {\sl local corrector} for monotonicity: an algorithm that takes some input $x$, makes queries to a black-box function $f$, and outputs $f_{mon}(x)$ where $f_{mon}$ is a monotone function that is close to $f$ in Hamming distance, if such a function exists. A local corrector, combined with any improper hypothesis, yields a proper hypothesis (similarly, a local corrector combined with a Hamming-distance test yields a tolerant test for monotonicity). The efficiency of the local corrector determines how quickly the proper hypothesis can be evaluated. The running time of our corrector is polynomial in the number of coefficients in the hypothesis of \cite{bshouty1996fourier}, the state-of-the-art improper learner for monotone functions. This allows their hypothesis to be made proper with a polynomial increase in its evaluation time. \\

\paragraph{Parallelizing greedy algorithms.} One of our core ideas is to bridge our learning task with a large body of work on \emph{parallelizing greedy algorithms}. [citations] 
Greedy algorithms are often useful for outputting one of many possible labelings on a large domain --- for example the indicator of a maximal independent set on a large graph. 
Such algorithms work as follows: choose some ordering on the vertices, and fix the label on each one conditioned on the labels of vertices that come earlier in the ordering. 
In a distributed setting, the goal is for each vertex to output its own label without needing to simulate all the vertices that come before it in the ordering. 
We call this ``parallelizing'' a greedy algorithm. 
We present a problem of this type for which a greedy algorithm is known, and a ``parallelized'' greedy algorithm would yield an efficient proper learner for monotone functions. 

\paragraph{The poset-sorting problem.} One of our core ideas is to bridge our learning task with a large body of work on parallelizing greedy algorithms in the setting of local and distributed computing. There exists a large body of work on this topic: see [] for an overview. (\cite{Ghaffari16} add references talk about MIS).
Specifically, we introduce the problem of {\em poset sorting}, that is, sorting binary values on a partially ordered set (poset), which we believe is of independent interest: 
\begin{center}
\textit{
Let $P$ be poset of $N$ elements with longest chain length at most $h$ and such that every element has at most $\Delta$ predecessors or successors. Given a binary labeling $f$ of elements of $P$, output a new binary labeling $f_\text{mon}$ that (i) is monotone with respect to the partial order in $P$ (ii) can be obtained from $f$ by a sequence of swaps of monotonicity-violating label pairs. 
}
\end{center}

Why is an algorithm for sorting on a poset $P$ relevant to proper learning? Suppose we obtained an improper predictor $f$ via the algorithm of \cite{bshouty1996fourier}, in the form of a circuit computing $f$. Then, let monotone $f_\text{mon}$ be obtained from $f$ by flipping a sequence of monotonicity-violating labels. It is not hard to argue that since $f$ was $O(\epsilon)$-close to the monotone $g$ we are trying to learn, then so is $f_\text{mon}$. Therefore, if we manage to transform the small circuit computing $f$ into a small circuit computing such $f_\text{mon}$, then proper learning is accomplished. 
What guarantee does one need from the sorting algorithm to accomplish such transformation? Roughly, one needs that to evaluate $f_\text{mon}$ at a given element $x$ the algorithm needs to compute $f$ on only a small number of points (and have an appropriately fast run-time). If we have a sorting algorithm satisfying this guarantee, then we can augment the circuit for $f$ with a circuit that executes this sorting algorithm, and as a result obtain a small circuit for $f_\text{mon}$. It turns out that problems about this exact type of guarantee have been studied in the so-called LCA (local computation algorithm) model. 

\paragraph{How we obtain an LCA for poset sorting problem.} 

Furthermore, it has been studied extensively how to implement various greedy algorithms in this model\footnote{This turns out to be intimately connected to implementing greedy algorithms in the distributed local model and in the massively parallel computation model}.     

\emph{parallelizing greedy algorithms}. [citations] 
Greedy algorithms are often useful for outputting one of many possible labelings on a large domain --- for example the indicator of a maximal independent set on a large graph. 
Such algorithms work as follows: choose some ordering on the vertices, and fix the label on each one conditioned on the labels of vertices that come earlier in the ordering. 
In a distributed setting, the goal is for each vertex to output its own label without needing to simulate all the vertices that come before it in the ordering. 
We call this ``parallelizing'' a greedy algorithm. 
We present a problem of this type for which a greedy algorithm is known, and a ``parallelized'' greedy algorithm would yield an efficient proper learner for monotone functions. 

An eye-catching property of the poset problem 



%Fortunately, algorithms satisfying this exact type of guarantee that is provided by the LCA (local computation algorithm) model.  


There is 


%A small circuit for the sorting problem then allows one to obtain a small circuit for such $f_\text{mon}$, without having to write out the whole function. This allows one to use $f_\text{mon}$ as a proper hypothesis. 



Thus, to accomplish our task we need an 

Clearly, there is a greedy algorithm for sorting that swaps monotonicity-violating pairs of labels until there are none left.
The challenge is to do this in a local fashion; i.e., to output the sorted label for a vertex without computing the entire sorted labeling.
Among the many distributed and parallel computation models, the one that is most relevant to us is the {\sl local computation algorithm} (LCA) model, defined formally in \cite{RTVX11, AlonRVX12}.
LCAs are well-studied in the literature on distributed and sublinear algorithms (some examples include
\cite{RTVX11, AlonRVX12,levi_local_2015, Ghaffari16,
reingold_new_2014, even_best_2014, ChangFGUZ19}).
In brief, to be an LCA, an algorithm should be local in the sense that it should not need to read the entire assignment of labels to vertices in order to determine which label will end up at some particular vertex $\vect{x}$. It should suffice to read only the labels of vertices that lie in a restricted neighborhood of $\vect{x}$ --- ideally not much more than the set of vertices one would need to read in order to determine whether $\vect{x}$'s own label violates monotonicity. We explain the algorithm itself in Subsection \ref{subsection: the algorithm summary}. \\

%As a result, the running time and query complexity of this algorithm depend primarily on $\Delta$ and $h$. 
%Specifically, in the LCA model of distributed computation, given query access to $P$ and $f$ we need to implement query access to  $f_\text{mon}$. 


\paragraph{Proper learning via local correction.} Why is an LCA for sorting on a poset $P$ relevant to proper learning? Suppose we obtained an improper predictor $f$ via the algorithm of \cite{bshouty1996fourier}. Then, let monotone $f_\text{mon}$ be obtained from $f$ by flipping a sequence of monotonicity-violating labels. It is not hard to argue that since $f$ was $O(\epsilon)$-close to the monotone $g$ we are trying to learn, then so is $f_\text{mon}$. An LCA then allows one to obtain a fast evaluator for such $f_\text{mon}$, without having to write out the whole function. This allows one to use $f_\text{mon}$ as a proper hypothesis. 
%\gray{Furthermore, this LCA allows one to obtain a tolerant tester for functions over general posets, rather than just the Boolean cube.}

In other words, an LCA for sorting on a poset is a {\sl local corrector} for monotonicity: an algorithm that takes some input $x$, makes queries to a black-box function $f$, and outputs $f_{mon}(x)$ where $f_{mon}$ is a monotone function that is close to $f$ in Hamming distance, if such a function exists. Local correctors for various function properties are studied in \cite{ACCL07, SS10} \textbf{todo: more cites on local correction}. A local corrector, combined with any improper hypothesis, yields a proper hypothesis. The efficiency of the LCA determines how quickly the proper hypothesis can be evaluated.

\paragraph{Tolerant monotonicity testing via local correction.}...\\


Stepping back, we give an application of LCAs to the setting of (centralized) PAC learning and tolerant testing --- a connection that is less discussed but we believe is quite natural. Efficient local correctors may exist for many function classes, and this connection may yield more algorithms for both learning and testing.


\subsection{Our LCA for sorting on a poset.}\label{subsection: the algorithm summary}

When the longest chain length $h$ is 1, this problem is equivalent to the classical problem of finding a maximal matching on a bipartite graph with $N$ vertices and maximum degree at most $\Delta$. We note that a recent LCA by Ghaffari and Uitto 
\cite{GhaffariU19} handles this problem using a run-time of $\Delta^{O(\log\log \Delta)}\polylog(N)$. \red{ Maybe emphasize here that Ghaffari and Uitto is a powerful result that followed a long line of research?}



For larger values of $h$, a naive approach would be to execute a sequence of phases, in each of which a maximal matching between monotonicity-violating labels is produced and the labels that are matched with each other are swapped. One can show that $O(h)$ such phases suffice and sometimes necessary if the matchings are arbitrary. If the algorithm of \cite{GhaffariU19} is used to implement each of the phases, this yields a run-time of $\left(\Delta^{O(\log\log \Delta)}\polylog(N)\right)^h$.
For properly learning monotone functions over the Boolean cube, the parameters\footnote{These are the parameters for small constant $\epsilon$. A slight subtlety in our argument is that we need to work over truncated hypercube, i.e. handle separately $O(\epsilon)$ fraction of the elements with too high or too low Hamming weight. This is a standard technique, and in our case it makes the parameter $\Delta$ in our poset small enough for us to get a good run-time guarantee using our poset sorting algorithm.
} we are primarily interested in are $h =\Theta(\sqrt{n})$, $\Delta = 2^{\tilde{\Theta}(\sqrt{n})}$ and $N=\Theta(2^n)$.
The naive approach then gives us a run-time of $\left(\Delta^{O(\log\log \Delta)} \polylog(N)\right)^h=2^{\Omega(n)}$, which is too slow for our purposes.

We beat the naive approach by enforcing that the maximal matchings at each step only include pairs of vertices that are sufficiently far away in the graph.
We show that after each matching step, the greatest distance between pairs that violate monotonicity reduces by a factor of 2. This allows us to reduce the exponent from $h$ to $\log h$, which is sufficiently fast to yield an essentially optimal proper learner for monotone functions. \\


%\gray{Our local corrector must sort labels in a truncated region of the Boolean cube, which is a poset of height $h = \tilde{O}(\sqrt{n})$ and $\Delta = 2^{\tilde{O}(\sqrt{n})}$. To give local access to the sorted configuration of labels in $2^{o(n)}$ time, we require a more general algorithm that scales well with $h$. To achieve an exponent of $\log h$ rather than $h$, we enforce that the maximal matchings at each step only include pairs of vertices that are sufficiently far away in the graph.} \\  

%How does such an algorithm help with proper learning of monotonicity? We may truncate the Boolean cube to only the vertices of Hamming weight $n/2 \pm \tilde{O}(\sqrt{n})$ and sort the labels in this truncated region. The sorting works by matching pairs of vertices that are sufficiently far from each other and whose labels violate monotonicity, and swapping them. We harness an efficient LCA for finding maximal matchings \cite{GhaffariU19}, which comes from a long line of work on parallelizing greedy graph algorithms [\textbf{todo: list of cites}]. The argument goes roughly as follows.  \\

%\gray{We show that the process of swapping labels between pairs that violate monotonicity cannot increase the Hamming distance between the function and any monotone function, and therefore cannot increase the error beyond the distance to monotonicity.} \\

\subsection{Other related work}
\textbf{todo: jane}
The problem of locally correcting monotonicity has been studied in \cite{ACCL07} and \cite{SS10}, in various parameter settings. The work of \cite{ACCL07} introduces the problem of online property reconstruction and gives an algorithm for this task for real-valued functions over the discrete numberline $[n]$. The work of \cite{SS10} introduces the framework of local property reconstruction, which is the same framework our approach uses (i.e., local correction by parallelizable LCA). They give a local corrector for functions over the hypergrid $[n]^d$, with large dependence on $d$ but small dependence on $n$.\\ 

Lower bounds: \cite{BGJ+10},
Parnas Ron Rubinfeld (introduced tolerant testing): \cite{Parnas2004TolerantPT},








==> local_corrector.tex <==

\section{The local corrector.}

The following is true from existing work:
\begin{theorem}
\label{theorem: LCA for maximal independent set}
For any positive constant $C$ the following is true.
Suppose we are given a graph of $N$ vertices with all vertex degrees at most $\Delta$, accessed via an adjacency list oracle (i.e. when queried $(v,j)$ with $v$ a vertex and $j$ an index, the oracle outputs the unique ID of the $j$-th neighbour of $v$, or $\perp$ otherwise). There is an LCA for computing a maximal independent set for this graph that requires $2^{\polylog (\Delta)}\,\polylog (N)$  oracle queries and run-time for each LCA query, with utilization of $2^{\polylog (\Delta)}\,\polylog (N)$ common randomness in total and success\footnote{In the context of LCAs, by the success probability we mean probability of \textbf{global} success of the algorithm. I.e. if one were to make every single query available, then the aggregate result thus obtained would satisfy the required specifications with given probability.} probability at least $1-\frac{1}{N^{C}}$.
\end{theorem}

\begin{corollary}
\label{corollary: can do local maximal matching}
For any positive constant $C$ the following is true.
Suppose we are given a graph of $N$ vertices (not necessarily bipartite) with all vertex degrees at most $\Delta$, accessed via an adjacency list oracle (i.e. when queried $(v,j)$ with $v$ a vertex and $j$ an index, the oracle outputs the unique ID of the $j$-th neighbour of $v$, or $\perp$ otherwise). Then, there is an LCA for computing a maximal matching\footnote{I.e. when the LCA is queried with an edge $(v_1,v_2)$ it has to answer whether it is to be included in the maximal matching. } for this graph that requires $2^{\polylog (\Delta)}\,\polylog (N)$  adjacency list oracle queries and run-time for each LCA query, with utilization of $2^{\polylog (\Delta)}\,\polylog (N)$  common randomness in total and success probability at least $1-\frac{1}{N^{C}}$.
\end{corollary}
\begin{proof}
Let $H$ be the following graph:
\begin{itemize}
    \item There is a vertex in $H$ for every edge in our original graph. In addition to these, there are $N$ extra vertices\footnote{We add these to boost success probability.}
    \item The added extra vertices have no edges adjacent to them.
    \item For two edges $e_1$ and $e_2$ in the original graph, there is an edge in $H$ between the vertices corresponding to $e_1$ and $e_2$ if and only if $e_1$ and $e_2$ share an endpoint in our original graph.
\end{itemize}

We observe that this resulting graph $H$ has at most $2N$ vertices and maximum degree at most $2\Delta$. Furthermore, we can simulate a single adjacency list query for $H$ using $O(\Delta)$ adjacency list queries to our original graph (all neighbours of a vertex $v$ in $H$ can be retrieved by  (i) first checking if it is any of the extra vertices and if so returning $\perp$ (ii) considering the endpoints of the edge corresponding to $v$ in our original graph (iii) using the adjacency list of our original graph to find all the edges adjacent to these neighbours in our original graph). 

We see immediately from definitions that a maximal independent set on $H$ corresponds to a maximal matching on our original graph. Since an adjacency list query on $H$ can be simulated with $O(\Delta)$ overhead via adjacency list queries on our original graph, we therefore get a maximal matching algorithm on our original graph using $\Delta\,2^{\polylog (O(\Delta))}\,\polylog (O(N))=2^{\polylog (\Delta)}\,\polylog (N)$  adjacency list oracle queries and run-time for each LCA query, with utilization of $2^{\polylog (\Delta)}\,\polylog (N)$  common randomness in total and success probability at least $1-\frac{1}{N^{C}}$.


\end{proof}
Now, consider a poset consisting of elements $\{v_i\}$, and we use the symbols $\prec$ and $\succ$ to denote dominance on the poset, as well as symbols $\precimm$ and $\succimm$ to denote immediate predecession and succession\footnote{$v_i\precimm v_j$ if  $v_i\prec v_j$ and there is no element of the poset $u$ satisfying $v_i\prec u \prec v_j$, conversely for $v_i\succimm v_j$}.

We consider the problem of locally correcting a function $f:\:\{v_i\}\rightarrow \{0,1\}$ to make it monotone. Specifically, we would like to provide local access to a monotone function $g$ such that\footnote{For $\{0,1\}$-valued functions $g_1$ and $g_2$, we use the notation $\norm{g_1-g_2}$ to denote the fraction of poset elements on which these two functions disagree.} 
\[
\norm{f-g}\leq O\left(\min_\text{monotone $h$}\norm{f-h}\right).
\]

Suppose the poset has $N$ elements and each element has at most $\Delta$ immediate predecessors and successors. We are given access to the poset via an adjacency-list-like oracle to the immediate predecessors and successors of a given poset element\footnote{It would make sense to also get a comparison oracle, but that seems that does not seem to be needed in the algorithm we are using.}. We are also given an oracle access to the function $f$ we would like to correct. The LCA would provide query access to a corrected function $g$.

Consider the following procedure (henceforth referred to as \textbf{the correcting procedure}) for a given parameter $r$:
\begin{itemize}
    \item Initialize $h_0=f$.
    \item For $i\in \{1,\cdots,r\}$ steps:
    \begin{itemize}
        \item Form a graph $G_i$ whose vertices are the poset elements, and edges are between pairs $v,u$ for which $v\precimm u$ but $h_i(v)=1$ and $h_i(u)=0$.
        \item Obtain a maximal matching $M_i$ over $G_i$.
        \item Form a function $h_{i+1}$ by:
        \begin{itemize}
        \item If an element $v$ of the poset has no edge in the matching $M_i$ adjacent to it, then $h_{i+1}(v)=h_i(v)$. 
            \item For every edge $(u,v)$ in the maximal matching in $G_i$, with $v\precimm u$ set\footnote{I.e. take the direct opposite of what $h_i$ was taking on these elements.} $h_{i+1}(v)=0$ and $h_{i+1}(v)=1$.
        \end{itemize}
    \end{itemize}
\item    Output the function $g=h_r$.
\end{itemize}

\begin{definition}
We say that the poset is $r$-good if irrespective of the initial $\{0,1\}$-valued function $f$ and the choice of matching in each step of the main loop of the algorithm above, the final function $g=h_r$ is monotone. 
\end{definition}

\begin{claim} For any positive constant $C$ the following is true.
It the setting explained above ($N$ total poset elements, at most $\Delta$ immediate predecessors and successors for each element), suppose the poset is $r$-good, and we are given oracle access to a function $f$ on the poset, as well as oracle access. Then there is an LCA that upon query gives oracle access to a monotone function $g$ over the poset for which
\[
\norm{f-g}\leq 2\min_\text{monotone $h$}\norm{f-h}.
\]
Furthermore, each LCA query
requires only $2^{r\,\polylog (\Delta)}\,(\polylog (N))^r$  oracle queries and run-time. In total, $r\,2^{\polylog (\Delta)}\,\polylog (N)$ bits of common randomness is utilized. Success probability is at least $1-\frac{r}{N^{C}}$.
\end{claim}
\begin{proof}
The algorithm simulates correcting procedure, while utilizing the maximal matching algorithm in Corollary \ref{corollary: can do local maximal matching} to compute the matching $M_i$ at each step. The probability that this local algorithm succeeds at all $r$ iterations is at least $1-\frac{r}{N^C}$, which we assume henceforth. As each iteration utilizes $2^{\polylog (\Delta)}\,\polylog (N)$  common randomness, the total amount of common randomness utilized is $r2^{\polylog (\Delta)}\,\polylog (N)$.

We first go about showing that the guarantee $\norm{f-g}\leq 2\min_\text{monotone $h$}\norm{f-h}$ will holds. Since the poset is $r$-good (and since the matching algorithm succeeds in all $r$ iterations), the resulting function $g$ will be monotone. Furthermore, one can get from $f$ to $g$ via flipping a sequence of violated immediate successor-predecessor pairs.\footnote{We say a successor-predecessor pair $(u,v)$ with $u\succimm v$ is violated for a function $h$ if $h(u)<h(v)$. To flip this pair means to change the function $h$ to a new function 
$h'(x)=\begin{cases}h(u)&\text{if $x=v$},\\
h(v)&\text{if $x=u$},\\
h(x)&\text{otherwise}
\end{cases}$.} This is true, because at each iteration of the algorithm a whole set of such successor-predecessor pairs are flipped in this manner (sequence of flipping does not matter as no two of these pairs share an element). 

Now, let $h^*\in \argmin_\text{monotone $h$}\norm{f-h}$ and Let $h_\text{track}$ track the function as it changes from $f$ to $g$ via flipping of violated successor-predecessor pairs. We observe as a successor-predecessor pair $(u,v)$ is flipped, the value of $\norm{h_\text{track}-h^*}$ can only decrease (this follows by recalling that $h^*$ is monotone and then considering all the possibilities for the pair of values $h^*$ takes on $u$ and $v$). Altogether, this means that $\norm{g-h^*}\leq \norm{f-h^*}$ which by triangle inequality implies $\norm{g-f}\leq 2\norm{f-h^*}=2\min_\text{monotone $h$}\norm{f-h}$ as required.

We claim one can compute a value of $h_{i+1}$ with $2^{\polylog (\Delta)}\,\polylog (N)$ queries to values of $h_i$ and run-time expenditure. Indeed:
\begin{itemize}
    \item For an edge $(v_1,v_2)$ (with $v_1\precimm v_2$) determining if it is in $G$ takes only two queries to $h_i$ (i.e. query $h_i(v_1)$ and $h_i(v_2)$ and say "yes" if $h_i(v_1)> h_i(v_2)$) .
    \item  To get all the neighbours of vertex $v$ in $G_i$, one can go through all (at most $2\Delta$) its immediate successors and predecessors (in the poset) and for each of them, determine if the edge connecting it with $v$ is in $G_i$. This takes $O(\Delta)$ queries to $h_i$. (Clearly, this  allows us to get the $j$-th neighbour of $v$ in $G$ as well for a given $j$.)
    \item To determine if an edge $(v_1,v_2)$ is in $M_i$ one needs at most $2^{\polylog (\Delta)}\,\polylog (N)$ adjacency list queries (of $G_i$) and run-time as per Corollary \ref{corollary: can do local maximal matching}. This boils down to $2^{\polylog (\Delta)}\,\polylog (N)$ run-time and queries to $h_i$ (the extra $O(\Delta)$ factor can be absorbed into the constant in the exponent).
    \item To determine the value of $h_{i+1}$ on a given vertex $v$, it is enough to query $h_i(v)$ and determine whether any of the (at most $2\Delta$) adjacent edges in is $M_i$. As per the previous bullet point, this takes $2^{\polylog (\Delta)}\,\polylog (N)$ run-time and queries to $h_i$ (again, the extra $O(\Delta)$ factor can be absorbed into the constant in the exponent).
\end{itemize}

Now, we come back to our original measure of resource consumption: total run-time together with oracle queries to $f$ and the immediate predecessor/successor oracle for the poset.
Clearly, computing a value of $h_0$ on a given element takes $O(1)$ oracle queries and run-time (since $h_0=f$. Therefore, computing a value of $h_i$ on a given element takes $2^{i\,\polylog (\Delta)}\,(\polylog (N))^i$ oracle queries and run-time, giving us the desired $2^{r\,\polylog (\Delta)}\,(\polylog (N))^r$ oracle queries and run-time bound for computing a value of $h_r$.

\end{proof}



==> path_shortening_lemma.tex <==

\section{Path shortening lemma}
%We have $\epsilon\in(0,1)$ and we assume it is sufficiently small. We let $H_n$ be the truncated hypercube 
%$$
%H_n:=\fig{\vect{x} \in \{0,1\}^n:~\abs{\sum_ix_i-\frac{n}{2}}\leq t},
%$$
%where $t:=\sqrt{\frac{n}{2}\log \frac{20}{\epsilon}}$. Via Hoeffding's bound, we have that the fraction of elements in $\{0,1\}^n$ that is not also in $H_n$ is at most $2\exp\left(-\frac{2t^2}{n}\right)=\frac{\epsilon}{10}$.

\begin{definition}[High-distance violation graph]
\label{def:viol-graph}
For a graded directed graph $G$ of height $h$, a function $f$ over $V(G)$, and some $d \in [h]$, we define the high-distance violation graph $G_d$ as follows:

\begin{itemize}
	\item $V(G_d) = V(G)$, and 
	\item For $\vect{u}, \vect{v} \in V(G)$, $(\vect{u}, \vect{v}) \in E(G_d)$ iff $\vect{u} \prec_G \vect{v}$, $\dist_G(\vect{u}, \vect{v}) \ge d$, and $f(\vect{u}) > f(\vect{v})$.
\end{itemize}
\end{definition}


\begin{lemma}[Distance shortening lemma]\label{lemma: path shortening lemma}
Let $P$ be a graded poset. 
Let $f$ be a $\{0,1\}$-valued function over $P$ and $k$ be a positive integer. Let $B_{k}$ be a graph whose vertex set is $P$ and two vertices $\vect{v}$ and $\vect{w}$ are connected when both of the following hold (i) $\vect{v}\prec \vect{w}$ and $f(\vect{v})>f(\vect{w})$ or $\vect{v}\succ \vect{w}$ and $f(\vect{v})<f(\vect{w})$ (ii) $\dist(\vect{v}, \vect{w}) \geq k$. Suppose one picks some maximal matching $M$ over $B_{k}$ and obtains a new function $f'$ as follows
$$
f'(x)=
\begin{cases}
f(x) &\text{if $x$ was not matched},\\
f(y) &\text{if $x$ was matched to some $y$}.
\end{cases}
$$
Then, we have
$$
\max_{\vect{v}, \vect{w} \in P: ~ \vect{v}\succ \vect{w},~ f'(\vect{v})=0 \text{ and } f'(\vect{w})=1  }\dist(\vect{v} , \vect{w}) \leq \max\left(k-1, \left(\max_{\vect{v}, \vect{w} \in P: ~ \vect{v}\succ \vect{w},~ f(\vect{v})=0 \text{ and } f(\vect{w})=1  }\dist(\vect{v} , \vect{w})\right) - k \right).
$$
\end{lemma}
\begin{proof}
Let $\lambda: P \rightarrow P$ map $\vect{x}$ to (i) $\vect{y}$ if $\vect{x}$ was mapped to some $\vect{y}$ by $M$ (ii) $\vect{x}$ itself otherwise. Note that $f'(\vect{x})=f(\lambda(\vect{x}))$ and also $\lambda$ is one-to-one. 

Let $x,y$ in $P$ be such that $\vect{x}\succ \vect{y}$, $f(\vect{x})=0$ and $f(\vect{y})=1$. If $\dist(\vect{x},\vect{y}) \geq k$, it cannot be the case that both $\lambda(\vect{x})=\vect{x}$ and $\lambda(\vect{y})=\vect{y}$, because then $M$ would not be a maximal matching since we could also match $\vect{x}$ to $\vect{y}$. Besides, note that if $\lambda(\vect{x}) \neq \vect{x}$ then $\lambda(\vect{x}) \prec \vect{x}$ and  $\dist(\vect{x},\lambda(\vect{x}))\ge k$. Analogously, if $\lambda(\vect{y}) \neq \vect{y}$ then $\lambda(\vect{y}) \succ \vect{y}$ and  $\dist(\vect{y},\lambda(\vect{y})) \ge k$. Additionally, for any $\vect{a},\vect{b},\vect{c}\in P$ if $\vect{a} \succ \vect{b} \succ \vect{c}$ then $\dist(\vect{a},\vect{c}) = \dist(\vect{a},\vect{b})+\dist(\vect{b},\vect{c})$.
Taking these observations together, we see that only following cases are possible
\begin{enumerate}
    \item $\dist(\vect{x},\vect{y}) \leq k-1$.
    \begin{enumerate}
        \item $\lambda(x) \succ \lambda(y)$ and $\dist(\lambda(\vect{x}),\lambda(\vect{y})) \leq \dist(\vect{x},\vect{y}) \leq k-1$.
        \item It is not the case that $\lambda(x) \succ \lambda(y)$.
    \end{enumerate}
    \item $\dist(\vect{x},\vect{y}) \geq k$.
    \begin{enumerate}
    \item $\lambda(\vect{x})=\vect{x}$ and $\dist(\vect{y},\lambda(\vect{y})\ge k$
    \begin{enumerate}
        \item $\lambda(x) \succ \lambda(y)$ and $\dist(\lambda(\vect{x}),\lambda(\vect{y}))\le \dist(\vect{x},\vect{y})-k$.
        \item It is not the case that $\lambda(x) \succ \lambda(y)$.
    \end{enumerate}
    \item $\lambda(\vect{y})=\vect{y}$ and $\dist(\vect{x},\lambda(\vect{x}))\ge k$
    \begin{enumerate}
        \item $\lambda(x) \succ \lambda(y)$ and $\dist(\lambda(\vect{x}),\lambda(\vect{y}))\le \dist(\vect{x},\vect{y})-k$.
        \item It is not the case that $\lambda(x) \succ \lambda(y)$.
    \end{enumerate}
    \item $\dist(\vect{x},\lambda(\vect{x}))\ge k$ and $\dist(\vect{y},\lambda(\vect{y}))\ge k$
    \begin{enumerate}
        \item $\lambda(x) \succ \lambda(y)$ and $\dist(\lambda(\vect{x}),\lambda(\vect{y}))\le \dist(\vect{x},\vect{y})-2k$.
        \item It is not the case that $\lambda(x) \succ \lambda(y)$.
    \end{enumerate}
    \end{enumerate}
\end{enumerate}
In the whole, if $\lambda(x) \succ \lambda(y)$ then $\dist(\lambda(\vect{x}),\lambda(\vect{y}))\leq \max(k-1,\dist(\vect{x},\vect{y})-k)$.

Now let's consider what happens after the swap. Let $\vect{v}_0,\vect{w}_0$ in $P$ maximize $\dist(\vect{v}_0,\vect{w}_0)$ subject to $\vect{v}_0\succ \vect{w}_0$, $f'(\vect{v}_0)=0$ and $f'(\vect{w}_0)=1$. Let $\vect{x}=\lambda^{-1}(\vect{v}_0)$ and $\vect{y}=\lambda^{-1}(\vect{w}_0)$.
Since $f'(\vect{v}_0)=0$, we have $\vect{x} \succeq \vect{v}_0$ and since $f'(\vect{w}_0)=1$, we have $\vect{y} \preceq \vect{w}_0$. Therefore, $\vect{x} \succ \vect{y}$. Also, $f(\vect{x})=f'(\vect{v}_0)=0$, $f(\vect{y})=f'(\vect{w}_0)=1$ and $\lambda(\vect{x})\succ\lambda(\vect{y})$. The conclusion of the previous paragraph tells us that $\dist(\vect{v}_0,\vect{w}_0)= \dist(\lambda(\vect{x}),\lambda(\vect{y})) \leq \max(k-1,\dist(\vect{x},\vect{y})-k)$. Overall,
\begin{multline*}
    \max_{\vect{v}, \vect{w} \in P: ~ \vect{v}\succ \vect{w},~ f'(\vect{v})=0 \text{ and } f'(\vect{w})=1  }\dist(\vect{v} , \vect{w}) =  \dist(\vect{v}_0,\vect{w}_0) \leq \max(k-1,\dist(\vect{x},\vect{y})-k) \leq\\
    \leq\max\left(k-1, \left(\max_{\vect{v}, \vect{w} \in P: ~ \vect{v}\succ \vect{w},~ f(\vect{v})=0 \text{ and } f(\vect{w})=1  }\dist(\vect{v} , \vect{w})\right) - k \right),
\end{multline*}
which finishes the proof.
\end{proof}

